Online Stochastic Bin Packing

Bin packing is an algorithmic problem that arises in diverse applications such as remnant inventory systems, shipping logistics, and appointment scheduling. In its simplest variant, a sequence of $T$ items (e.g., orders for raw material, packages for delivery) is revealed one at a time, and each item must be packed on arrival in an available bin (e.g., remnant pieces of raw material in inventory, shipping containers). The sizes of items are i.i.d. samples from an unknown distribution, but the sizes are known when the items arrive. The goal is to minimize the number of non-empty bins (equivalently waste, defined to be the total unused space in non-empty bins). This problem has been extensively studied in the Operations Research and Theoretical Computer Science communities, yet all existing heuristics either rely on learning the distribution or exhibit $o(T)$ additive suboptimality compared to the optimal offline algorithm only for certain classes of distributions (those with sublinear optimal expected waste). In this paper, we propose a family of algorithms which are the first truly distribution-oblivious algorithms for stochastic bin packing, and achieve $\mathcal{O}(\sqrt{T})$ additive suboptimality for all item size distributions. Our algorithms are inspired by approximate interior-point algorithms for convex optimization. In addition to regret guarantees for discrete i.i.d. sequences, we extend our results to continuous item size distribution with bounded density, and also prove a family of novel regret bounds for non-i.i.d. input sequences. To the best of our knowledge these are the first such results for non-i.i.d. and non-random-permutation input sequences for online stochastic packing.

==> tex/PD_departures.tex <==
\section{Dynamic Bin Packing} \label{sec:PD_departures}

In this section we discuss stochastic online bin packing when items arrive and depart over time. As described in Section \ref{sec:model}, we assume that items arrive according to a Poisson process with rate $\lambda$, their types are sampled i.i.d. from a distribution $F$, and their sojourn time in the system are exponentially distributed with means given by $M = \{\mu_1, \ldots, \mu_{J}\}$. We will be concerned with the number of open bins in steady-state as a function of arrival rate $\expct{N_F(\lambda)}$. Our research effort had started with the question: \emph{Is Best Fit optimal for stochastic dynamic bin packing?} In our working paper \cite{GuptaRadovanovic2012}, we provided experimental evidence indicating that the answer in general is: \emph{no}. In Section~\ref{sec:PD_departures_simple} we prove that under our Primal-Dual algorithm, and without congestion dependent slowdown, the system state converges on a `fluid scale' to a packing which uses $OPT\times(1+\epsilon)+o(\lambda)$ bins for arbitrary $\epsilon > 0$. 

In Section~\ref{sec:PD_departures_heterogeneous} we consider the general version where the departure rate of a type $j$ item in configuration $c$ is slowed down (or sped up) to $\mu_j s_{c,j}$. This scenario highlights the advantage of a Lagrangian based approach to online packing, and we propose an algorithm based on the complete Lagrangian (that is, not partially Lagrangifying the non-negativity constraints alone) using a trick we call proxy duals. We provide experimental evidence for its asymptotic optimality.
% but where the number of items of different types are sampled from the steady-state distribution (it is easy to establish that the number of type $j$ items in steady-state will have a Poisson distribution with mean $\lambda p_j m_j$, independent of number of items of other types).

%In Section~\ref{sec:PD_departures_homogeneous}, we consider the slightly general case where items experience congestion-dependent slowdown, but the slowdown is homogeneous within a configuration. That is, $s_{cj}=s_c$. For this case, we propose a generalization of the PD heuristic, and provide some analytic justification of its optimality.


\subsection{Primal-Dual algorithm under item departures} \label{sec:PD_departures_simple}
Our proposed PD algorithm extends almost as-is to the case of item departures. As before we define configuration potentials as:
\[ V_c(t) \doteq  1 - \kappa e^{-\epsilon(t) N_c(t)}\]
where $N_c(t)$ is influenced by departures as well, and an arrival of type $j$ at time $t$ is placed in configuration $c^*$ to create $c^* +e_j$ where
\[ c^* = \argmin_{c:N_c(t)>0} V_{c +e_j}(t) - V_c(t).\]
Experimentally we have observed $\tilde{O}(\sqrt{\lambda})$ additive suboptimality when setting $\epsilon(t) = \sqrt{\frac{|\mC|}{2(|\mC| +N(t))}}$, where $N(t)$ denoting the total number of items in the system, but is it extremely hard to prove convergence under this setting. % since the different components of the state vector evolve at different scales -- and there is no easy Lyapunov function to analyze the system.
Instead, we prove a weaker optimality guarantee by setting $\epsilon(t) = \frac{1}{\epsilon \lambda}$ for a small enough $\epsilon$ ($\lambda$ can be replaced by $N(t)$), and analyzing our system under fluid scaling. In this case, the Lagrangian $\mL(N(t))$ acts as a Lyapunov function.

\begin{theorem} In the absence of congestion-dependent slowdown, Primal-Dual algorithm with $\epsilon(t) = \frac{1}{\epsilon \lambda}$, and $\kappa>2$ is asymptotically $(1+\mO(\epsilon))$ competitive for steady-state mean number of bins used for any $\epsilon > 0$. 
\end{theorem}
The proof details are in Appendix~\ref{sec:proofs_PD_departure_simple}.


%\subsubsection{Optimality Analysis}




\subsection{Packing with slowdowns: The Proxy Dual method} \label{sec:PD_departures_heterogeneous}
In this section we consider the still more general problem of congestion-dependent slowdowns: the departure rate of a type $j$ item in configuration $c$ is given by $\mu_j s_{cj}$. Our convention will be $s_{e_j, j} = 1$, that is the slowdown of an item type when it is the only item in a bin is the benchmark of slowdown. Due to lack of space, we only describe the algorithm, and a simulation experiment. See Appendix~\ref{sec:proxy_dual_details} for more details.

\begin{figure}[h!]
\fbox{\begin{minipage}{0.95 \columnwidth}{
\textbf{Algorithm PD$_{\mbox{het}}$} : 
\begin{itemize}[itemsep=0pt]
\item Define configuration duals: $ \alpha_c(t) = 1 - \kappa e^{-\epsilon(t) N_c(t)}$
where $\kappa \geq m \cdot \max_{c, k,k' \in c} \frac{s_{ck'} }{s_{ck}}$ ($m$ denotes the maximum number of items in any configuration).
\item Define configuration potentials: $ V_c(t) = (1 - \alpha_c(t)) - \sum_{j} x_{cj}s_{cj} (1-\alpha_{e_j}) $
with $V_\emptyset \doteq 0$. 
\item Place arriving item, say of type $j$, in configuration $c^*$ to create $c^* \cup j$, where:
\[ c^* = \argmin_{c: N_c(t) > 0} V_{c +e_j}(t) - V_{c}(t) \]
\end{itemize}
}
\end{minipage}}
%\caption{Primal-Dual algorithm for heterogeneous slowdowns}
\label{alg:PD_heterogeneous}
\end{figure}

Figure~\ref{fig:PDhet_transient} shows a simulation sample path for the transient behavior of PD$_{\mbox{het}}$ heuristic on an instance with $B=9$, items of sizes $2,3$ and randomly generated slowdowns $\{s_{cj}\}$. The distribution $F$ undergoes two changes, at times $t=20$ and $t=40$. The fluid scale convergence to optimality as well as $o(\lambda)$ suboptimality in steady-state is quite evident. A formal proof of asymptotic optimality of PD$_{\mbox{het}}$ is under preparation.

\begin{figure*}
\centering
\subfigure[$\lambda = 10^4$]{
\includegraphics[height=1.9in]{PD_het_transient_sim_lambda_10e4}
}
\subfigure[$\lambda = 10^5$]{
\includegraphics[height=1.9in]{PD_het_transient_sim_lambda_10e5}
}
\caption{\small Simulation results comparing transient behavior of PD$_{\mbox{het}}$ algorithm against the LP optimal. The Bin size is $B=9$, with items of size $2,3$. The distribution changes from $F=\{p_2=0.5,p_3=0.5\}$ to $F=\{p_2=0.3, p_3=0.7\}$ at $t=20$, and then to $F=\{p_2=0.7, p_3=0.3\}$ at $t=40$. The service rates $M = \{\mu_2 = 2.408,\mu_3=1.643\}$ were randomly generated. All the slowdowns were randomly sampled from $U[0.1,1]$.}
\label{fig:PDhet_transient}
% simulation data for $\lambda=10^4$ is snapshotted in simulation_for_PD_het_transient_sim_lambda_10e4.mat (in the MATLAB folder)
\end{figure*}


==> tex/PD_nodepartures.tex <==
\section{Static Bin Packing} \label{sec:PD_nodepartures}

In this section we propose a scheme for stochastic online bin packing without item departures that achieve additive $\mO(\sqrt{n})$ suboptimality for $i.i.d.$ item sizes irrespective of the distribution $F$. As mentioned before, there is no simple, {\it distribution-oblivious} bin packing heuristic known that performs optimally in the case of linear waste distributions. In this setting it was shown that the Sum-of-Squares (SS) heuristic achieves constant factor larger waste than the optimal. All attempts to improve this performance so far have relied on the knowledge of distribution $P_F$ (\cite{SumOfSquares_JACM_CsirikJKOSW06}, \cite{courcoubetis1986necessary}) or its learning in the process of packing (\cite{RheeTalagrand93}). Further, there are no heuristics for packing in the configuration model. Our algorithm fills this gap.

\subsection{`Patching' the Sum-of-Square Rule for LW distributions}\label{sec:PDquad_informal}
We first describe two simple tweaks to the SS rule that can give $\mO(\sqrt{n})$ suboptimality for all distributions (see working paper \cite{GuptaRadovanovic2012} for further discussion). It turns out that the resulting algorithm is a special case of the penalized-Lagrangian algorithm, which we describe subsequently. \\
Recall that in trying to minimize $\sum_{h=1}^{B-1}N_h^2$, SS tries to equalize the number of bins of each level. This heuristic works for perfectly packable distributions where the items can be packed without any $N_h$ growing large. However, for LW distributions some $N_h$ must grow as $\Theta(n)$, and SS heuristic `pulls along' the number of bins which have room for more items. E.g., for $B=5$ and only size 2 items, SS creates $\Theta(n)$ bins of level 4 as well as 2.

There seems to be an easy fix to this problem: Since we want to control our heuristic using a sum-of-square potential term, we do not want any $N_h$ to grow as $\Theta(n)$. Therefore, we allow bins to be started at any level $h$, creating forbidden holes at the bottom of some bins. But this change alone does not work. Nothing now prevents us from opening a new bin for each item and sending them to level $B-j$. We fix this by penalizing items which cause the level of a bin to reach $B$! Therefore, on the arrival of $t$th item of size $s$, we send it to level $h^*$ where
\[ h^* = \argmin_{h}  \left[ C \cdot \mathbf{1}_{h=B-s} +  N_{h+s}(t-1) - N_h(t-1) \right] \]
where $C$ is the penalty amount. We can equivalently view this heuristic as minimizing the cost function:
\begin{align*}
L(\mathbf{N}) &= C \cdot N_{B} + \frac{1}{2} \sum_{h=1}^{B-1} N_h^2
\end{align*}
which is a combination of the Best Fit and SS cost functions (but still rather odd due to penalty for `full bins'). In the next section we formalize this idea as gradient descent on a penalized partial Lagrangian of the bin packing LP and present the optimality results.

\subsection{Bin-packing LP and Primal-Dual algorithms}

Given the item size distribution $F$, the optimal \emph{bin rate} for $F$ (that is, the average number of bins used per item) can be computed by solving the following Linear Program (called the configuration LP):
\begin{align*}
b(F) &= \min_{n_c} \sum_{c \in \mC} n_c & \mathbf{(P_{static})}\\
\mbox{subject to } \quad &  \forall c \in \mC \ : \ n_c \geq 0 \\
 & \forall j \in [J] \ : \ \sum_{c} n_c x_{cj}  = p_j
\end{align*}

The variables $n_c$ denote the expected number of configuration $c$ bins opened per item from $F$. (In the working paper \cite{GuptaRadovanovic2012}, we had looked at the 1-d level packing problem via \emph{flow LP} which is a more compact representation than the configuration LP).\\
 Our approach is quite straightforward in hindsight: Rather than learn the distribution $F$ and then solve the configuration LP, our packing heuristic mimics online saddle point optimization of the Lagrangian of the bin packing LP with stochastic gradients (the stochasticity coming from the random arrival of items) via \emph{Primal-Dual} iteration. However, we do not explicitly maintain dual variables, instead mapping the primal state of the packing to duals -- and thus our algorithm in fact bears closer resemblance to interior point methods.  We begin with a general template for design of Primal-Dual algorithms to build intuition, and then present our algorithm and guarantees formally.%incrementally move towards the optimal Given the simplicity and convergence properties of the primal-dual method for solving LPs, we propose a simple algorithm that would 

\subsubsection{A general template for Primal-Dual algorithms}
Consider the following convex problem:
\[ \mbox{minimize} \   f(x) \ ,  \qquad \mbox{subject to} \ g(x) \leq 0. \]
The approach of penalized-Lagrangian optimization is to convert the constrained optimization problem into an unconstrained optimization by imposing a strictly convex increasing penalty function on the constraint and moving this penalty into the objective function:
\[ \mbox{minimize} \quad \mathcal{L}(x) =  f(x) + \Phi(g(x))\]
Further, given the optimal solution $x^*$ to the above optimization problem, an approximation to the value of the dual $\lambda_g$ for the constraint $g(x) \leq 0$ can be obtained by comparing the two forms
\begin{align*}
\left[ \grad{f} +  \frac{\partial \Phi(g)}{\partial g} \cdot \grad g \right]_{x^*} = 0
\quad \mbox{and} \quad 
\left[ \grad{f} +  \lambda_g \cdot \grad g \right]_{x^*} = 0
\end{align*}
as $\lambda_g \approx \left. \frac{\partial \Phi(g)}{\partial g} \right|_{g(x^*)}$. Now depending on our choice of penalty function $\Phi(\cdot)$, there is a full menu of Lagrangian relaxations, each with its own mapping of primal to dual variables:
\begin{itemize}
\item Quadratic: $\mathcal{L}_{\mbox{\footnotesize quad}}(x) = f(x) + \frac{1}{2\epsilon}\left( g(x)^+ \right)^2$ \hspace{1in} Dual: $\lambda_g = \frac{g(x)^+}{\epsilon}$\\
For the dual variables to drive the algorithm, we \emph{must violate the primal constraints}. %That is, we always have a primal infeasible solution. Primal-dual heuristics with quadratic penalty are common in controlling queueing systems (e.g., \cite{TassiulasEphremides92, Stolyar2005}) because queues are nothing but temporary violations of capacity constraints and map to the corresponding duals. In \cite{GuptaRadovanovic2012}, we had discussed the packing algorithm corresponding to quadratic penalty applied to the flow LP, which interestingly packs bins in a top-down fashion. 
The heuristic in Section \ref{sec:PDquad_informal} corresponds to using quadratic penalty with flow LP for 1-d packing, and packs bins in a top-down fashion (see \cite{GuptaRadovanovic2012}).
We will not discuss this variant here.
\item Translated Quadratic: $\mathcal{L}_{\mbox{\footnotesize tquad}}(x) = f(x) + \frac{1}{2\epsilon}\left( (g(x)+\eta)^+ \right)^2$  \hspace{1in} Dual: $\lambda_g = \frac{(g(x)+\eta)^+}{\epsilon}$\\
A small variation over Quadratic penalty which allows duals to be non-zero even when the constraint is satisfied, but yields zero duals when constraints are $\eta$-far from violation.
\item Exponential penalty: $\mathcal{L}_{\mbox{\footnotesize exp}}(x) = f(x) + \epsilon \cdot e^{\frac{g(x)}{\epsilon}}$ \hspace{1in} Dual: $\lambda_g = e^{\frac{g(x)}{\epsilon}}$ \\
The dual variables are always non-zero even when the primal solution is feasible. Exponential duals are very popular for worst-case (non-stochastic) online packing and covering problems (e.g., \cite{AwerbuchKhandekar08, PlotkinShmoysTardos95, BuchbinderJainNaor07}, and in prediction with experts' advice. Our PD heuristic is precisely the Lagrangian relaxation of the configuration LP with exponential penalty. This method also corresponds to Online Mirror Descent algorithm for solving the dual maximization problem with entropy as the mirror map function (a.k.a., distance generating function). 
\item $\log$-barrier: $\mathcal{L}_{\log}(x) = f(x) - \epsilon \cdot \log( - g(x))$  \hspace{1in} Dual: $\lambda_g = -\frac{ \epsilon}{g(x)}$\\
The solution is constrained to be always primal feasible, and $\log$ is a self-concordant barrier function which offer provable convergence guarantees for Newton-Raphson iteration. Therefore they are often used in interior point algorithms for convex optimization \cite{BoydVandenberghe}. %This would indeed give us another Primal-Dual bin packing variant, but currently we can not prove a better than $O(\sqrt{n \log n})$ additive suboptimality using $\log$-barrier. This agrees with the results on regret in online convex optimization where the diameter of the primal space under the regularization function (rather the Bregman distance corresponding to the regularizer) shows up in the regret term. The diameter of the $\log$ function is  $\log n$, while the exponential function is bounded between $[0,1]$ over the space $0 \leq N_c \leq n, \forall c$.
\end{itemize}
In each case, as $\epsilon \to 0$, the penalty function approaches the barrier penalty, and $\epsilon$ controls the violation of constraints (for quadratic penalty), or the loss in objective function (for exponential and $\log$-barrier).

\subsection{The Primal-Dual algorithm for algorithm for bin packing}
We define the partial penalized-Lagrangian using the exponential penalty function for non-negativity constraints:
\[ \mL(t) = \sum_c N_c(t) + \frac{\kappa}{\epsilon(t)} \sum_c e^{-\epsilon(t) N_c(t)}.\] 
The PD algorithm is a greedy minimization of the above penalized-Lagrangian. Noting that $\frac{\del \mL(t)}{\del N_c(t)}=1-\kappa e^{-\epsilon(t)N_c(t)}$:

\begin{figure}[h!]
\fbox{\begin{minipage}{0.95 \columnwidth}{
\textbf{Algorithm PD} : At time $t$
\begin{itemize}
\item Define configuration potentials: $ V_c(t) = 1 - \kappa e^{ -\epsilon(t) N_c(t)}$ \\
with $V_\emptyset \doteq 0$.
\item Place arriving item, say of type $j$, in configuration $c^*$ to create $c^* + e_j$, where:
\[ c^* = \argmin_{c: N_c(t)>0} V_{c +e_j}(t) - V_{c}(t) \]
\end{itemize}
}
\end{minipage}}
\end{figure}

We first analyze the case where we know the total number of arrivals $n$ and $\epsilon(t)$ is fixed, and then the more general case when $n$ is not known (\emph{open-ended} algorithm) and $\epsilon(t)$ varies with $t$.

\begin{theorem}\label{thm:PDexp_fixed_epsilon}
For the PD-exp algorithm with $\epsilon(t) = \sqrt{\frac{|\mC|}{n}}$ and $n>|\mC|$,
\[ \expct{N_F^{\mbox{\footnotesize PD}}(n)} \leq \expct{N_F^{OPT}(n)} + \sqrt{4 |\mC|n } .\]
\end{theorem}

\begin{theorem}\label{thm:PDexp_varying_epsilon}
For the PD-exp algorithm with $\epsilon(t) = \sqrt{\frac{|\mC|}{2(|\mC|+t)}}$,
\[ \expct{N_F^{\mbox{\footnotesize PD}}(n)} \leq \expct{N_F^{OPT}(n)} + \sqrt{8 |\mC| (n+|\mC|)} .\]
\end{theorem}

The proofs are rather simple potential function analysis, and appear in Appendix~\ref{sec:proofs}. A simple application of Azuma-Hoeffding inequality extends our bounds on expected suboptimality to concentration bounds.

\begin{theorem}[Martingale concentration] \label{thm:martingale} For a packing problem with horizon $n$, for all $t$:
\[ \prob{\sum_c N_c(t) \geq t b(F) +  \sqrt{|\mC|t} + \sqrt{|\mC|n} +  \sqrt{ 2 \lambda \delta t \log t} } \leq \frac{1}{t^\lambda} .\]
where $\delta \leq 4 + \frac{\sqrt{|\mC|}}{2}$.
\end{theorem}

\subsection{Bounded inventory guarantees}
The Primal-Dual algorithm described in the previous section keeps all bins open (potentially $\Omega(n)$ many), which might be undesirable. We now prove that if instead of $\mO(\sqrt{n})$ regret, we only desire $(1+\epsilon)$ competitive ratio, then $\mO\left(\frac{1}{\epsilon}\right)$ open bins suffice with translated-quadratic penalty based Lagrangian.

Define the class of \emph{$\eta$-bounded per-configuration inventory algorithms}: $\widetilde{N}_c(t)$ denotes the number of configuration $c$ bins in inventory,  each $\widetilde{N}_c$ is capped at $\eta$. If a configuration $c$ bin is created at time $t+1$ when $\widetilde{N}_c(t) = \eta$ then the new bin is considered closed. The number of open bins is bounded by $\eta|\mC|$ at all times.

\begin{theorem}[Bounded inventory]\label{thm:bounded_upperbound} The $\eta$-bounded per-configuration inventory Primal-Dual algorithm using translated quadratic penalty function:
\[  \mL_{\mbox{\footnotesize tquad}}(N,\widetilde{N}) = \sum_c N_c + \frac{1}{2}\epsilon \sum_c \left( \eta- \widetilde{N}_c  \right)^2 \]
with per configuration inventory $\eta = \frac{1}{\epsilon}+1$ is asymptotically $(1+\mO(\epsilon))$ competitive.
\end{theorem}

We use quadratic penalty function above because with exponential penalty function we require $\Omega\left(\frac{1}{\epsilon} \log \frac{1}{\epsilon} \right)$ inventory. The next theorem proves that in the general case, we must keep $\Omega\left(\frac{1}{\epsilon} \right)$ bins open.

\begin{theorem}\label{thm:bounded_lowerbound} For the 1-dimensional bin packing instance with $B=3$, and items of size $1$ and $2$ with probability $\frac{1}{2}$ each, any online algorithm with a bound of $I$ on the number of open bins must have asymptotic competitive ratio of at least $\left(1+ \frac{1}{9I}\right)$.
\end{theorem}


\subsection{Guarantees against non-i.i.d. input}
From the proof of Theorem~\ref{thm:PDexp_fixed_epsilon}, it is easy to obtain the following corollary for an adversarial setting where an adversary may choose a different distribution $F_t$ at each time step : Let the item at time step $t$ be generated from an arbitrary distribution $F_t$ chosen by an adversary, possibly after observing the packing decisions in the first $(t-1)$ time steps. If the optimal bin-rate of $F_t$ is $b_t$ then the proposed PD algorithm achieves: $ \expct{N_{\{F_t\}}^{PD}(n) } \leq \sum_{t=1}^n b_t + \mO(\sqrt{n}) $.

How good is the above guarantee? Consider the case where $B=3$, and an adversary alternately and deterministically sends items of sizes $1$ and $2$. The bin-rate of the former distribution is $1/3$ and for the latter is $1$, giving an average of $2/3$. However, it is conceivable that we should be able to achieve the optimal bin-rate of $1/2$ given the benign nature of input. As we show, we indeed have such a stronger guarantee against a \emph{smoothed} input sequence, albeit at a slightly worse additive suboptimality.

We first formally define the model of generating sequences:\\
\textbf{Adversarial Model:} At time $t$, the adversary samples an item type $S_t$ from distribution $F_t$ that is a function of the history of samples generated by him: $F_t = f_t(S_1, \ldots, S_{t-1}).$ Let $ \left\{ \mathcal{F}_t \right\}$ denote the filtration generated by $\{ S_1, \ldots, S_t \}$ where as is usual $\mathcal{F}_0 = \{\emptyset, \Omega\}$.
%\begin{remark} We could allow the adversary to sample items based on the actions of the PD algorithm until time $t-1$, since the PD algorithm is deterministic and therefore the adversary could simulate the actions of the PD algorithm. However, for randomized algorithms, we want the algorithm to have access to private randomness. Further, the adversarial model above allows analysis of algorithms with lookahead window of $L$ by forcing the adversary to commit to the next $L$ time steps, although we do not perform this analysis here. \end{remark}

\begin{theorem} \label{thm:adversarial_smoothed}
Consider a packing horizon of $n$ items and the adversarial arrival model described above. Consider an arbitrary conditioning time $t$.  For a given window size $L$, define the \emph{$L$-smoothed arrival distribution} at time $k$ conditioned on $\mathcal{F}_t$ as:
\[ 
\hat{F}_{L,k|t} \doteq  \expct{ \left. \frac{1}{L} \sum_{m=k}^{k+L-1} F_m  \right| \mathcal{F}_t}
\]
Denote the optimal bin-rate of the bin packing LP for $\hat{F}_{L,k|t}$ by $\hat{b}_{L,k|t}$. For succinctness, $\hat{b}_{L,k} \doteq \hat{b}_{L,k|0}$. Let $\epsilon$ and $\kappa$ denote the parameters of the exponential Lagrangian function. 

If $L, \epsilon, \kappa, |\mC|$ satisfy: $\epsilon L < 1$, and $L \leq \frac{1}{\epsilon} \log \frac{\kappa |\mC|}{|\mC|-1}$, then:
\[ \expct{ N^{PD}(n) | \mathcal{F}_t } \leq \sum_{k=1}^n \hat{b}_{L,k|t} +  n \kappa \epsilon \left( \frac{2L+3}{4} \right) + \frac{|\mC| \kappa }{\epsilon} + L. \]
\end{theorem}

The proof of Theorem~\ref{thm:adversarial_smoothed} appears in Appendix~\ref{sec:proofs}. The main idea is to perform a potential function argument over a random time distributed uniformly in $[t,t+L-1]$. This ensures that the arrival is from the smoothed distribution. However, the arriving job now sees a random packing instead of a deterministic packing, which may potentially be correlated with the type of the arriving item. Since the support of the random time is bounded, the support of the packings is ``narrow'', which allows us a graceful increase in suboptimality. %This argument is similar in spirit to the one carried out by Neely \cite{Neely2009} for Markov chain controlled environment. However, there the author considers a deterministically delayed Lyapunov function to allow the environment at time $t$ to ``de-correlate'' with the state at time $t-L$, and then using the fact that state at time $t$ is ``$L$-close'' to the state at time $t-L$.

\begin{corollary} \ 
%\label{cor:fix_alpha}
\begin{enumerate}
\item Fixing $\epsilon=\Theta(n^{-1/2})$ and $L = O(n^{c})$ for any $c<\frac{1}{2}$: $ \expct{N^{PD}(n) } \leq \sum_{k=1}^n \hat{b}_{L,k} + O(n^{\frac{1}{2}+c}). $

\item %\label{cor:vary_alpha}
If $L = \Theta(n^{c})$  ($0 \leq c < 1$), choosing $\epsilon = \Theta(n^{-\frac{1+c}{2}})$: $ \expct{N^{PD}(n) } \leq \sum_{k=1}^n \hat{b}_{L,k} + O(n^{\frac{1+c}{2}}). $
\end{enumerate}
\end{corollary}

As an application, consider an adversary who fixes a distribution $F$ (with bin rate $b(F)$) and then generates a sequence of $n$ i.i.d. samples from it. He then shuffles this sequence, but never moving any item more than $W/2$ places from its original position. With a smoothing window of size $L$, the smoothed distribution has bin rate $b(F) + \mO(\frac{W}{L})$. Therefore, knowing $W$ and fixing $L= n^{1/3}W^{2/3}$ (and hence $\epsilon = \Theta(n^{-2/3}W^{-1/3})$) in part 2 of the corollary, we get a regret of $\mO(n^{2/3}W^{1/3})$ for any $W=o(n)$ against offline optimal. If $W = o(\sqrt{n})$ but unknown, then setting $\epsilon=\Theta(n^{-1/2})$ gives a regret of $\mO(n^{3/4}W^{1/2})$ (set $L=n^{1/4}W^{1/2}$ in part 1 of the corollary).



==> tex/PDconv.tex <==
\subsection{Proof of Theorem \ref{thm:PDquad_convergence}}
\label{sbsec:pdconv}

In the chosen example, the steady state number of items is distributed as Poisson random variable with mean $\lambda$, and the initial configuration to PD-quad places all these in bins with a hole of size 1 at the bottom. We now show that if we fix a random bin which is initially in this configuration, then it takes $\Omega{\sqrt{\frac{\lambda}{\log \lambda}}}$ time in expectation for this bin to empty, and thus for PD-quad to recover the forbidden hole of size 1. In fact, we will prove that it takes this time in expectation for this bin to first reach a state with only two size 1 items.

As before, let $N_h(t)$ denote the number of level $h$ bins at time $t$. We first make the following claim on the supremum of $N_h(t)$. The claim follows from known results on the supremum of mean-reverting stochastic processes (Ornstein-Uhlenbeck process), and we omit it for clarity.

\begin{claim}
Over a time interval of length $\poly(\lambda)$, the supremum of $N_h(t)$ ($1 \leq h \leq 4$) is bounded above by $\alpha \sqrt{\lambda \log \lambda}$ for some constant $\alpha > 0$ with probability $1-\frac{1}{\poly(\lambda)}$.
\end{claim}

We now condition on the event of the above claim, and the mean time until a bin with four items first reaches a state with two items. Let $T_{4\to 3}$ denote the mean time until a this bin of level 5 with four items first reaches level 4 with three items, and let $T_{3 \to 2}$ denote the mean time until a bin of level 4 with three size one items reaches level 3. Due to our assumptions of Poisson arrivals and i.i.d. exponential residence times of jobs, the system evolves according to a Markov chain. It is easy to see that 
\[T_{4 \to 3} = \frac{1}{4} \]

Now when the bin reaches level $4$, it either has a departure which happen at rate $3$ to become a level $3$ bin, or an external arrival increases the level of this bin to 5. The crucial observations are
\begin{itemize}
\item $N_4(t)$ is upper bounded by $\alpha \sqrt{\lambda \log \lambda}$
\item since level 4 bins are created at a rate of $\lambda$ due to departure from level 5 bins, they also get destroyed at rate $\lambda$ due to external arrivals wich increase their level to 5
\end{itemize}
Since an arrival picks a level 4 bin at random (conditioned on the arrival choosing a level 4 bin), our tagged bin gets picked with probability at least $\frac{1}{\sqrt{\lambda \log \lambda}}$. Therefore, the rate at which this bin sees an arrival to become a level 5 bin is at least $\sqrt{\frac{\lambda}{\log \lambda}}$. We now write the recurrence for $T_{3 \to 2}$:
\begin{align*}
T_{3 \to 2} & \geq \frac{1}{3 + \sqrt{\lambda / \log \lambda} } + \frac{\sqrt{\lambda / \log \lambda}}{3 + \sqrt{\lambda / \log \lambda}} \cdot (T_{4 \to 3} + T_{3 \to 2}) \\
\intertext{or,}
T_{3 \to 2}& \geq \frac{1}{3} + \sqrt{\lambda / \log \lambda} \frac{T_{4 \to 3}}{3} \\
&= \frac{1}{3} + \frac{1}{12} \sqrt{\frac{\lambda}{ \log \lambda}} 
\end{align*}


==> tex/PDopt.tex <==
\section{Proofs}
\label{sec:proofs}

\subsection{Optimality Analysis of the Primal-Dual Algorithm with Quadratic Penalty Function}
\label{sbsec:quadratic} 

\paragraph{Proof of Theorem~\ref{thm:PDquad_fixed_epsilon}} \ \\
Recall that we cast our algorithm as the minimization of the following Lagrangian:
\begin{align*}
L(\mathbf{N}) &= \underbrace{B \cdot N_B - (\mbox{total volume of jobs seen})}_{F_{A}(t)} + \epsilon \cdot \underbrace{\frac{1}{2} \sum_{h=1}^{B-1} N_h(t)^2}_{V_{A}(t)},
\end{align*}
where the second term represents the quadratic relaxation of the penalty paid for violating constraint (\ref{eqn:constr_destr}), and $N_h\equiv N_h(t)$, $1\leq h\leq B$, denote the number of bins at level $h$, where $\mathbf{N}=(N_1,N_2,\dots, N_{B})$. We call the first term, $F_{A}$, the primal objective function value, and the second term, $V_{A}$, the potential function value for algorithm $A$.

We first note that we can bound the waste of any algorithm $A$ at time $t$ as 
\begin{align}
\label{eq:partialw}
W_A(t) \leq F_A(t) + B \sum_{h=1}^{B-1} N_h(t).
\end{align}

Next, note that $N_h\le B^2/\epsilon$, $1\le h\le B-1$, since one can always send an incoming item $j$ to level $B-s_j$, while paying $B-\epsilon N_{B-s_j}$, which is less then $B$. Therefore, since for all $h_1$, $h_2$, $N_{h_1}-N_{h_2}\le B$, we obtain $N_h\le B^2/\epsilon$, $h=1,\dots, B-1$, which implies that the waste due to partially filled bins is at most $\frac{B^4}{2\epsilon}$. 

Next, we show that
\begin{align}
\expct{F_{PD}(n)} \leq \expct{F_{OPT}} + \epsilon n 
\end{align}
By choosing $\epsilon = \frac{B^2}{\sqrt{2n}}$, we then establish additive $\sqrt{n}$ waste of the PD algorithm. Since the PD algorithm minimizes the increase in the Lagrangian at each time step:
\begin{align*}
\Delta F_{PD}(t) + \epsilon \Delta V_{PD}(t) &\leq \Delta F_{OPT}(t) + \epsilon \Delta V_{OPT}(t)
\end{align*}
where $\Delta$ changes are evaluated with respect to the state at time $t$ and $OPT$ is some algorithm which we use as the representative of the optimal algorithm. Taking a telescoping sum of the above inequality gives us:
\begin{align*}
F_{PD}(n) - F_{OPT}(n) & \leq \epsilon [ V_{OPT}(n)  -V_{OPT}(0) ] - \epsilon [V_{PD}(n) - V_{PD}(0)] \\
& \leq \epsilon(V_{OPT}(n) + V_{PD}(0))
\end{align*}
assuming that $V$ is non-negative, which it is. Intuitively, the previous inequality implies that our algorithm performs well for the Lagrangian compared to $OPT$. However, our goal is to show that the primal objective value $F_{PD}$ is close to optimal. This happens if the OPT algorithm has not accumulated too much potential. 

In order to relate $F_{PD}(n)$ to the optimal waste of the waste LP (\ref{eq:primal}), $W_F$, we modify the policy $A_F$ defined in \cite{SumOfSquares_JACM_CsirikJKOSW06} to prove the performance of SS for Perfectly packable distributions.
\begin{definition}[$A_F$ policy (Csirik et al. \cite{SumOfSquares_JACM_CsirikJKOSW06})]
Given a bin $Y$ in the perfect packing $P^*$ and the current arbitrary packing $P$, we first find an ordering $y_1,y_2,\ldots, y_{|Y|}$ of the items in $Y$, and a threshold index $last(Y), \ 0 \leq last(Y) < |Y|$, such that if we set $S_i \equiv \sum_{j=1}^{i} s(y_j)$, then:
\begin{itemize}
\item $P$ has partially filled bins with each level $S_i$, $0 \leq i \leq last(Y)$
\item $P$ has no partially filled bins with level $S_{last(Y)} + s(y_i)$ for any $i > last(Y)$
\end{itemize}
Then, if the arriving item has index $j$ in the ordering of items in bin $Y$ and $j>last(Y)$, it is sent to a partially full bin at level $S_{last(Y)}$ (or $0$ if $last(Y)=0$). Otherwise, if $1< j\le last(Y)$, we place the item into a bin of level $S_{i-1}$. Finally, if $j=1$, we create a new bin with level $s(y_1)$.
\end{definition}

We now define our modification:
\begin{definition}[Modified $A_F$ policy for PD-quad]
Given a bin $Y$ in the optimal packing $P^*$ with a hole of size $s(-1)$ ($s(-1)=0$ for perfectly packed $Y$) and the current arbitrary packing $P$, we first find an ordering $y_1,y_2,\ldots, y_{|Y|}$ of the items in $Y$, and a threshold index $last(Y), \ 0 \leq last(Y) < |Y|$, such that if we set $S_i \equiv s(-1) + \sum_{j=1}^{i} s(y_j)$ ($S_{0}=0$), then:
\begin{itemize}
\item $P$ has partially filled bins with each level $S_i$, $0 \leq i \leq last(Y)$
\item $P$ has no partially filled bins with level $S_{last(Y)} + s(y_i)$ for any $i > last(Y)$
\end{itemize}
Then, if the arriving item has index $j \geq 1$ in the ordering of items in bin $Y$ and $j>last(Y) > 0$, it is sent to a partially full bin at level $S_{last(Y)}$.
\emph{If $last(Y)=0$ or $j=1$, the item is placed in a new empty bin at level $s(-1)$ to create a bin of level $s(-1)+s(y_j)$.}
 Otherwise, if $1 < j \le last(Y)$, we place the item into a bin of level $S_{j-1}$.
\end{definition}


% (An identical policy was used in \cite{SumOfSquares_JACM_CsirikJKOSW06} to prove the performance of the Sum of Squares packing algorithm for perfectly packable distributions.)  

Next, we show the following result:
\begin{proposition}
Given an arbitrary packing $P$, the probability that $A_F$ packs an item to close a bin (create a level $B$ bin) is at most the probability that a random item in the optimal packing $P^*$ is placed on the top of its bin.
\end{proposition}
\begin{proof}
For every bin $Y$ of $P^*$, $A_F$ first creates an ordering of items. Note that for any bin $Y$ in $P^*$, each item is randomly generated with equal probability. Now, if $A_F$ sees an item of size $s$ and it maps it to bin $Y$, then it can only create a level $B$ bin if it was the topmost item in the ordering. There is still a chance that it does not create a level $B$ bin because no bin of level $B-s$ exists. Since, in general, $F$ is not perfectly packable, we simply look at the optimal packing $P^*$, and for any bin which is not fully (perfectly) packed in the optimal packing configuration, $A_F$ pretends that it sees a bigger item of size equal to the item placed on the top plus the hole.
\end{proof}

Now, in view of the previous conclusions, we have
\begin{align*}
\Delta F_{PD}(t) + \epsilon \Delta V_{PD}(t) &\leq \Delta F_{A_F} + \epsilon \Delta V_{A_F},
\end{align*}
which, after taking expectations, yields
\begin{equation*}
\expct{\Delta F_{PD}(t)} -\expct{\Delta F_{A_F}(t)} \leq \epsilon \expct{\Delta V_{A_F}} - \epsilon \expct{ \Delta V_{PD}}.
\end{equation*}
Then, since $\expct{\Delta V_{A_F}}\le 1$ as proved in \cite{SumOfSquares_JACM_CsirikJKOSW06} (this property also holds for the modified $A_F$), we obtain
\begin{equation*}
\expct{\Delta F_{PD}(t)} - [B \cdot p_F - \expct{s_F}] \leq  \epsilon - \epsilon \expct{\Delta V_{PD}},
\end{equation*}
where $p_F$ is the rate at which OPT creates bins, and $s_F$ is the expected job size under $F$. Finally,
\begin{equation*}
\expct{F_{PD}(n)} - n \cdot W_F \leq \epsilon n + \epsilon \expct{V_{PD}(0)}.
\end{equation*}
By selecting $\epsilon = \Theta(\frac{B^2}{\sqrt{2n}})$ and adding the waste due to the partially full bins, we obtain an overall additive waste of $\sqrt{2B^4n}$.
\qed


\paragraph{Proof of Theorem~\ref{thm:PDquad_varying_epsilon}}\ \\
The proof of Theorem~\ref{thm:PDquad_fixed_epsilon} can easily be modified to show that when $\epsilon(t) = \frac{B^2}{\sqrt{4t}}$, we still get $O(\sqrt{n})$ waste, which ensures performance guarantees in the case where there is no knowledge of time horizon $n$. From (\ref{eq:partialw}) we get that the waste originating from the partially full bins can be bounded by $B^4/2\epsilon(n)=B^2\sqrt{n}$.

%nhe result about the $N_h$ being bounded by $\frac{B^2}{\epsilon(n)}$ still holds.
Similarly as before, at any time $t$, we have:
\begin{align*}
\Delta F_{PD}(t) + \epsilon(t) \left( V_{PD}(t)-V_{PD}(t-1) \right) &\leq \Delta F_{OPT}(t) + \epsilon(t) \left( V_{OPT}(t) - V_{OPT}(t-1) \right).
\end{align*}
By taking the telescoping sum of the previous inequalities for $0\le t\le n$, we obtain:
\begin{align*}
F_{PD}(n) - \sum_t \Delta F_{OPT}(t) &\leq \sum_{t=1}^{n} \epsilon(t) [ V_{OPT}(t)  -V_{OPT}(t-1) ]\\
& \quad + \sum_{t=1}^{n-1} V_{PD}(t) (\epsilon(t+1) - \epsilon(t)) +\epsilon(1) V_{PD}(0) - \epsilon(n) V_{PD}(n),
\end{align*}
which, after taking expectations, noting that $\epsilon(t)$ is decreasing, and replacing $\epsilon(t) = B^2/\sqrt{4t}$, yields
\begin{align}
\expct{F_{PD}(n)} - n \cdot W_F & \leq \sum_{t=1}^{n} \epsilon(t) + \epsilon(1) V_{PD}(0) - \epsilon(n) V_{PD}(n)\nonumber\\
& \leq 1 + \int_{1}^n \epsilon(t) dt + \epsilon(1) V_{PD}(0)\nonumber  \\
& \leq B^2 \sqrt{n} + V_{PD}(0).\nonumber
\end{align}
Thus, by adding the waste originating from the partially full bins, we obtain that the total additive waste is bounded by $\sqrt{4B^4n}$.

\subsection{Optimality Analysis of the Primal-Dual Algorithm with Exponential Potential Function}
\label{sbsec:exponential}

\paragraph{Proof of Theorem~\ref{thm:PDexp_fixed_epsilon}} \ \\
In this case, the Lagrangian function takes the following form:
\begin{align*}
L(\mathbf{N}(t)) &= \underbrace{\sum_{h=1}^{B-1} (B-h) N_h(t) }_{F_A(t)} + \underbrace{ \frac{1}{\epsilon_1} \sum_{h=1}^{B-1} e^{-\epsilon_2 N_h(t) } }_{V_A(t)},
\end{align*}
implying that its change per a single item placement can be bounded as
\begin{align}
\Delta L(\mathbf{N}) & \leq \sum_{h=1}^{B-1} (B-h) \sgn{\Delta N_h}  -\sum_{h=1}^{B-1} e^{-\epsilon_2 N_h } \left[ \frac{\epsilon_2}{\epsilon_1} \sgn{\Delta N_h} - \frac{\epsilon_2^2}{\epsilon_1}  \right]\label{eq:changeLag}
\end{align}
Our goal is to find a policy for which the change in primal as well as the potential term is small. The first means that a desirable policy should open a new bin with a probability not larger than the long run rate, irrespective of the state. Small increase in the potential term means that we prefer creating bins of some level rather than destroying them. 

Next, we consider a different modification to policy $A_F$ described in Subsection \ref{sbsec:quadratic}. If the bin $Y$ of optimal packing $P^*$ is perfectly packed, then we follow the $A_F$ as described originally by Csirik et al. If the bin $Y$ is non-full, then we modify $A_F$ as follows:
\begin{quote}
Given a non-full bin $Y$ in the optimal packing $P^*$ and the current arbitrary packing $P$, we first find an ordering $y_1,y_2,\ldots, y_{|Y|}$ of the items in $Y$, and a threshold index $last(Y), \ 0 \leq last(Y) \leq |Y|$, such that if we set $S_i \equiv \sum_{j=1}^{i} s(y_j)$, then:
\begin{itemize}
\item $P$ has partially filled bins with each level $S_i$, $0 \leq i \leq last(Y)$
\item $P$ has no partially filled bins with level $S_{last(Y)} + s(y_i)$ for any $i > last(Y)$
\end{itemize}
\end{quote}
That is, we allow $last(Y)$ to be equal to $|Y|$. Remaining definition is unchanged.

The change in the Lagrangian (\ref{eq:changeLag}) after a placement of an item with the ordering index $j$ can be upper bounded depending on the case: 
\begin{itemize}
\item If $j > last(Y)$ : an item is sent to a partially full bin at level $S_{last(Y)}$ (or 0 if $last(Y)=0$). This seems like a bad case because we destroy bins of some level with a higher probability than we create it, and that increases our potential function (unlike for SS potential). Also, if $last(Y)=0$, then we open new bins with probability higher than OPT. However, the crucial observation is that in this process we create a bin of some level which does not exist yet. This causes sufficiently large drop in the potential to completely annihilate the increase in primal term or the potential term for $S_{last(Y)}$. We differentiate between two subcases:
\begin{itemize}
\item $last(Y) = 0$:
\begin{equation*}
\Delta L \leq -s(y_j) + B + \frac{1}{\epsilon_1} (e^{-\epsilon_2} - 1) = -s(y_j) + B - \frac{\epsilon_2}{\epsilon_1} \left(1 - \frac{\epsilon_2}{2!} + \frac{\epsilon_2^2}{3!} - \ldots \right),
\end{equation*}
implying that for $\epsilon_2 < 1$
\begin{equation*}
\Delta L \leq  -s(y_j) + B - \frac{\epsilon_2}{\epsilon_1} \left( 1 - \frac{\epsilon_2}{2}  \right) = -s(y_j) + B - \frac{\epsilon_2}{\epsilon_1} + \frac{\epsilon_2}{\epsilon_1} \cdot \frac{\epsilon_2}{2},
\end{equation*}
which in conjunction with $\epsilon_2 = B\epsilon_1$ yields
\begin{equation*}
\Delta L \leq -s(y_j) +   \frac{B}{2} \epsilon_2.
\end{equation*}
\item $last(Y) > 0$ : we send an item to a bin with level $ h = S_{last(Y)} > 0$ with $n_h > 0$, implying the change in the potential function, i.e.
\begin{equation*}
\Delta L \leq -s(y_j) - \frac{1}{\epsilon_1} \left[ \left(1 - e^{-\epsilon_2} \right) - \left(e^{- n_h \epsilon_2} - e^{-(n_h-1) \epsilon_2 }\right)  \right]\leq -s(y_j)
\end{equation*}
\end{itemize}
\item $ 1 \leq j \leq last(Y)$ : one of these items causes a new bin to open and increase the objective function term by $B-s(1)$, while the others change the objective function by $-s(y_j)$. We now focus on the change in the potential function due to bins of level $S_1, \ldots, S_{last(Y)-1}$. We do not need to look at $S_{last(Y)}$ since $j=last(Y)$ only causes this number to increase and hence potential to fall, and we have already accounted for the effect of $j>last(Y)$ on the Lagrangian. Focusing on this set of items, the probability of the increase of $N_{S_i}$ is at least as much as the probability of decrease of $N_{S_i}$. Therefore, the expected change in the potential function due to level $S_i$ is at most (let $N_{S_i}=n$ before arrival of the tagged item):
\begin{align*}
\Delta V_i &  \leq \frac{1}{2\epsilon_1} \left[ \left( e^{-(n+1)\epsilon_2} - e^{-n \epsilon_2} \right)  + \left(e^{-(n-1)\epsilon_2} - e^{-n \epsilon_2} \right) \right] \\
&= \frac{e^{-n \epsilon_2}}{2\epsilon_1} \left[ e^{-\epsilon_2} + e^{\epsilon_2} - 2  \right] = \frac{e^{-n \epsilon_2}}{\epsilon_1} \left[ \frac{\epsilon_2^2}{2!} + \frac{\epsilon_2^4}{4!} + \frac{\epsilon_2^6}{6!} + \ldots  \right],
\end{align*}
implying
\begin{equation*}
\Delta V_i \leq  \frac{\epsilon_2^2}{\epsilon_1}\;\;\text{for $0<\epsilon_2<1$,}
\end{equation*}
and 
\begin{equation*}
\Delta V_i \leq  B \epsilon_2\;\;\text{for $\frac{\epsilon_2}{\epsilon_1} = B$.}
\end{equation*}
\end{itemize}

Now we look at the telescoping sum of changes in the Lagrangian:
\begin{equation}
\label{eq:relateWs}
\Delta F_{PD}(t) + \Delta V_{PD}(t) \leq \Delta F_{A_F} + \Delta V_{A_F},
\end{equation}
which after taking expectations yields
\begin{equation*}
\expct{\Delta F_{PD}(t)} \leq \expct{\Delta F_{A_F}(t)} + \expct{\Delta V_{A_F}} - \expct{ \Delta V_{PD}},
\end{equation*}
or
\begin{equation*}
\expct{\Delta F_{PD}(t)} \leq [B \cdot p_F - \expct{s_F}] +  B \epsilon_2 - \expct{\Delta V_{PD}},
\end{equation*}
where, similarly as before, $p_F$ is the rate at which OPT creates bins and $s_F$ is the expected job size under $F$. After summing across time horizon $1\le t\le n$, we obtain
\begin{equation}
\label{eq:sumEXP}
\expct{F_{PD}(n)} \leq n \cdot W_F + B n \epsilon_2 + \expct{V_{PD}(0)}
\end{equation}
and
\begin{equation*}
\expct{F_{PD}(n)}  \leq n \cdot W_F + B n  \epsilon_2 + \frac{B-1}{\epsilon_1}.
\end{equation*}
Assuming that $\epsilon_2 = B \epsilon_1$ and $\epsilon_1 = \sqrt{\frac{1}{Bn}}$, we derive
\begin{equation*}
\expct{F_{PD}(n)}  \leq n \cdot W_F + 2 \sqrt{B^3 n},
\end{equation*}
where $W_F$ is optimal value of the waste LP.

\paragraph{Proof of Theorem~\ref{thm:PDexp_varying_epsilon}} \ \\
The proof carries through similarly as in (\ref{eq:relateWs}) - (\ref{eq:sumEXP}) with minimal changes in the last step. Changes in the potential term of the PD algorithm do not telescope any more. In particular, the potential function keeps decreasing since $\epsilon(t)$ decreases. Note that in this case, we fix $\epsilon_2(t) = \epsilon(t)$ and $\epsilon_1(t)=\epsilon(t)/B$.

The sum of potential differences $\sum \Delta V_{PD}(t)$ equals to:
\begin{align*}
\sum \Delta V_{PD}(t) &= B \sum_{h=1}^{B-1} \sum_{t=1}^{n} \frac{1}{\epsilon(t)} (e^{-\epsilon(t)n_h(t)} - e^{-\epsilon(t)n_h(t-1)}) \\
&=  B \sum_{h=1}^{B-1}\left[ \frac{e^{-n_h(n) \epsilon(n)}}{\epsilon(n)} - \frac{e^{-\epsilon(0)n_h(0)}}{\epsilon(0)} + \sum_{t=1}^{n-1} \left( \frac{1}{\epsilon(t)} e^{ -\epsilon(t) n_h(t)} - \frac{1}{\epsilon(t+1)} e^{-\epsilon(t+1)n_h(t)} \right) \right].
\end{align*}
Since the second summand in the previous expression is minimized when $n_h(t) = 0$, we obtain
\begin{equation*}
\sum \Delta V_{PD}(t) \geq B \sum_{h=1}^{B-1}\left[  - \frac{e^{-\epsilon(0)n_h(0)}}{\epsilon(0)} + \sum_{t=1}^{n-1}\left( \frac{1}{\epsilon(t)} - \frac{1}{\epsilon(t+1)} \right) \right],
\end{equation*}
which, after selecting $\epsilon(t) = \frac{k}{\sqrt{t+a}}$, implies
\begin{equation}
\label{eq:boundPOT}
\sum \Delta V_{PD}(t) \geq -\frac{B(B-1)}{k}\left [\sqrt{a}  + \sum_{t=1}^{n-1} (\sqrt{t+1+a}-\sqrt{t+a}) \right] \geq - B(B-1) \frac{\sqrt{a+n}}{k}.
\end{equation}

Next, (\ref{eq:sumEXP}) and $\epsilon_2(t) = \epsilon(t)/B$ imply
\begin{align*}
&\sum\expct{\Delta F_{A_F} + \Delta V_{A_F} - W_F}\le B\sum_t \epsilon(t) = B\sum_{t=1}^{n} \frac{k}{\sqrt{t+a}}\\
&\le Bk\left (\frac{1}{a+1}+\int_{x=a+1}^{n=a}\frac{dx}{\sqrt{x}}\right)\\
&=Bk\left(\frac{1}{\sqrt{a+1}}+2\sqrt{n+a}-2\sqrt{a+1}\right)\le 2Bk\sqrt{n+a}.
\end{align*}
Therefore, the previous expression and (\ref{eq:boundPOT}) give an upper bound for the overall additive waste
\begin{equation*}
2Bk\sqrt{n+a} + B(B-1)\frac{n+a}{k},
\end{equation*}
which, by setting $k=\sqrt{B/2}$ and $a=B$, guarantees $\epsilon_2(t)<1$ and 
\begin{equation*}
\expct{F_{PD}(n)}\le n\cdot W_F + \sqrt{8B^3(n+B)}.
\end{equation*}


\subsection{Proof of Theorem \ref{thm:PDquad_convergence}}
\label{sbsec:pdconv}

In the chosen example, the steady state number of items is distributed as Poisson random variable with mean $\lambda$, and the initial configuration to PD-quad places all these in bins with a hole of size $1$ at the bottom. We now show that if we fix a random bin which is initially in this configuration, then it takes $\Omega\left ({\sqrt{\frac{\lambda}{\log \lambda}}}\right )$ time in expectation for this bin to empty, and, thus, for the PD-quad algorithm to recover the forbidden hole of size $1$.

As before, let $N_h(t)$ denote the number of level $h$ bins at time $t$. We first make the following claim on the supremum of $N_h(t)$. The claim follows from known results on the supremum of mean-reverting stochastic processes (Ornstein-Uhlenbeck process), and we omit it for clarity.

\begin{claim}
Over a time interval of length $\poly(\lambda)$, the supremum of $N_h(t)$ ($1 \leq h \leq 4$) is bounded above by $\alpha \sqrt{\lambda \log \lambda}$ for some constant $\alpha > 0$ with probability $1-\frac{1}{\poly(\lambda)}$.
\end{claim}

Next, we lower bound the mean time it takes a level $5$ bin with four items to reach the state with only two items conditioned on the event of the claim. Let $T_{4\to 3}$ denote the mean time until this bin reaches level 4 with three items, and let $T_{3 \to 2}$ denote the mean time it reaches level 3 with 2 items. Since the arrivals are Poisson and residence times i.i.d. and exponential, the system evolves according to a Markov chain. 

It is easy to see that
\[T_{4 \to 3} = \frac{1}{4}. \]
When the bin reaches level $4$, it transitions to a level $3$ bin (with rate $3$) in case of a departure, or to a level $5$ bin in case of an external arrival. The crucial observations are
\begin{itemize}
\item $N_4(t)$ is upper bounded by $\alpha \sqrt{\lambda \log \lambda}$;
\item Since level 4 bins are created at rate $\lambda$ due to departures from level 5 bins, they also get destroyed at rate $\lambda$ due to external arrivals wich increase their level to 5.
\end{itemize}
Since an arrival picks a level 4 bin at random (conditioned on the arrival choosing a level 4 bin), our tagged bin gets picked with probability at least $\frac{1}{\alpha\sqrt{\lambda \log \lambda}}$. Therefore, the rate at which this bin sees an arrival to become a level 5 bin is at least $\frac{1}{\alpha}\sqrt{\frac{\lambda}{\log \lambda}}$. We now write the recurrence for $T_{3 \to 2}$:
\begin{align*}
T_{3 \to 2} & \geq \frac{1}{3 + \sqrt{\lambda /\alpha^2 \log \lambda} } + \frac{\sqrt{\lambda /\alpha^2 \log \lambda}}{3 + \sqrt{\lambda /\alpha^2 \log \lambda}} \cdot (T_{4 \to 3} + T_{3 \to 2}) \\
\intertext{or,}
T_{3 \to 2}& \geq \frac{1}{3} + \sqrt{\lambda /\alpha^2 \log \lambda} \frac{T_{4 \to 3}}{3} \\
&= \frac{1}{3} + \frac{1}{12} \sqrt{\frac{\lambda}{ \alpha^2 \log \lambda}} .
\end{align*}

Therefore, for any bin of the initial configuration, it takes $\Omega\left(\sqrt{\frac{\lambda}{\log \lambda}} \right)$ time to empty out, and hence the waste under the PD-quad algorithm remains linear for at least $\Omega\left(\sqrt{\frac{\lambda}{\log \lambda}} \right)$ time.


==> tex/config.tex <==
\section{Configuration Model for Bin Packing}
\label{sec:config}
In this section we present a generalization of the one-dimensional model described in Section~\ref{sec:model} to configuration model. The flexibility of  configuration model allows modeling multi-dimensional bin packing and vector packing problems, as well as minimum cost packing. We briefly define the configuration model in Section~\ref{sec:confModel} and the extension of our algorithm to this setting in Section~\ref{sec:PDconf}.

\subsection{Model definitions}
\label{sec:confModel}

As before, item types $Y_t$ are $i.i.d.$ samples from  $ [J] = \{1,\dots,J\}$, with $p_j$ denoting the probability of type $j$. We abbreviate $F=\{p_1,\ldots, p_J\}$. Unlike one-dimensional level model where packing constraints were implicitly dictated by bin capacity and item sizes, here the set of feasible configurations is explicitly defined and denoted by $\mC$. Each $c\in \mC$ is represented by $x_{c} = (x_{c1}, \ldots, x_{cJ}) \in \N^{J}$. The quantity $x_{cj}$ represents the number of type $j$ items in configuration $c$.
We assume that the set $\mC$ is downward closed: if $c \in \mC$, then all $c'$ with $x_{c'j} \leq x_{cj}$ $\forall j $ are in $\mC$ as well. (The model can be extended to allow heterogeneous bins; we omit it for brevity).  We denote the empty configuration by $\emptyset$, the configuration with a single type $j$ item by $e_j$,  and $c + e_j $ and $c - e_j$ denote configurations with one more and one less item $j$, respectively (assuming they are in $\mC$). We denote the number of configuration $c$ bins in packing $P$ by $N_c(P)$, and with abuse of notation $N_c^A(t)$ will denote the number of bins in configuration $c$ after $t$th item has been packed by algorithm $A$. \\
The performance metric that we want to minimize is the number of bins opened by $A$ :
\begin{align*}
N(P) \triangleq \sum_{c \in \mC \backslash \emptyset }  N_c(P).
\end{align*}
For the minimum cost packing problem, we associate a weight $w_c$ to configuration $c$ bins and define the weight of a packing $P$ by:
\[ W(P) \triangleq \sum_{c \in \mC} w_c N_c(P) .  \]
As earlier, $P^A_F(T)$ denotes the packing after applying algorithm $A$ to $T$ items generated from $F$, and the expected costs $\expct{W_F^A(T)}$ and $\expct{N^A_F(T)}$ are defined analogously to \eqref{eqn:1dwaste}-\eqref{eqn:1dcost}. Note that the minimization problems for $N(P)$ and $W(P)$ are not equivalent unless $w_c$ satisfy: $c = q c_1 + (1-q) c_2$ implies $w_c = q w_{c_1} + (1-q) w_{c_2}$. To keep exposition simple, we will focus on the metric of minimizing total number of bins in this section.

\subsection{Bin packing Linear Program}
\label{sec:PDconf}

Analogous to $\mathbf{P_{1d-level}}$, we begin with a Linear Program that given the item type distribution $F$ finds the optimal number of bins per item for $F$:
\begin{align*}
b(F) &= \min_{ \{n_c\}_{\mC}} \sum_{c \in \mC} n_c & \mathbf{(P_{conf})}\\
\mbox{subject to } \quad &  \forall c \in \mC \ : \ n_c \geq 0 \\
 & \forall j \in [J] \ : \ \sum_{c} n_c x_{cj}  = p_j
\end{align*}

The variables $n_c$ denote the expected fractional number of configuration $c$ bins opened per item from $F$, and the non-negativity constraints ($n_c \geq 0$) are analogous to {\it (no floating items)} constraints in $\mathbf{P_{1d-level}}$. The second set of constraints are the mass balance constraints.

%%%%%%%%%%%%%%%%%%%
%%%%% BEGIN COMMENT
%%%%%%%%%%%%%%%%%%%
%% POSSIBLE ADD BACK LATER
\begin{comment}
Introducing dual variables $\alpha_c$ for the first set of non-negativity constraints, and $z_j$ for the second set of mass conservation constraint, we can write the following dual problem:
\begin{align*}
 & \max_{ \{z_j\}_{[J]} , \{\alpha_c\}_{\mC} } \sum_{j \in [J]} p_j z_j & \mathbf{(D_{conf})}\\
\mbox{subject to } \quad &  \forall c \in \mC \ : \ \alpha_c \geq 0 \\
 & \forall c \in \mC \ : \ \sum_{j} z_j x_{cj}  = 1 - \alpha_c
\end{align*}
\end{comment}
%%%%%%%%%%%%%%%%%%%
%%%%% END COMMENT
%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%
%%%%% BEGIN COMMENT
%%%%%%%%%%%%%%%%%%%
\begin{comment}
Note that it is possible to eliminate the duals $\alpha_c$ from the above dual program, but we have preserved them on purpose since $\alpha_c$ duals are the key to our algorithm. In fact, we will further write the following dual function parametrized by the $\{\alpha_c\}_\mC$ :
\begin{align}
\label{eqn:dualfunction}
q(\alpha) &= \sum_j p_j \min_{a_j \in A_j} \sum_c (1-\alpha_c) a_{jc}
\end{align}
Here the set $A_j \subset \{-1,0,+1\}^{|\mC|}$ is the set of feasible placement vectors for item type $j$: $A_j = \{ e_{c}-e_{c-e_j} | x_{cj} > 0  \}$ (with abuse of notation we use $e_c$  to denote a vector that is 1 for configuration $c$ and 0 everywhere else, and $e_j$ to denote a vector that is 1 for item type $j$ and 0 everywhere else). Equation~\eqref{eqn:dualfunction} can alternately be written in a less cumbersome but also less useful manner as:
\begin{align}
\label{eqn:dualfunction2}
q(\alpha) &= \max_{ \{z_j\}_{[J]}} \sum_j p_j  z_j   \\
\nonumber \mbox{ subject to } \quad & \forall c \in \mC \ : \ \sum_{j} z_j x_{cj} \leq 1-\alpha_c
\end{align}

Before proceeding we make a few observations: ($i$) The optimal solution of $\mathbf{D_{conf}}$ and hence $\mathbf{P_{conf}}$ is convex in $F = \{p_1,\ldots, p_J\}$. This implies $\expct{N^{OPT}_F(T)} \geq T \cdot b(F)$. ($ii$) $b(F) = \max_{\{\alpha_c\}_\mC} q(\alpha)$ where the latter maximization problem is concave. 
\end{comment}

%%%%%%%%%%%%%%%%%%%
%%%%% END COMMENT
%%%%%%%%%%%%%%%%%%%


\subsection{Primal-Dual algorithm}
Starting from $\mathbf{P_{conf}}$ the penalized Lagrangian where we dualize the $n_c>0$ constraints using exponential penalty function is given by:
\[ \mL_{exp}(n) = \sum_c n_c + \kappa \epsilon \sum_c e^{ - n_c /\epsilon}  .\]
As in Section~\ref{sec:PDlevel}, $n_c \sim \frac{N_c(t)}{t}$, giving:
\[ \mL_{exp}(N(t)) = \sum_c N_c(t) + \frac{\kappa}{\epsilon(t)} \sum_c e^{ - \epsilon(t) N_c(t)  } . \]

Finally, we obtain Algorithm~\ref{alg:PDexp} with the following performance guarantee. We omit the proof since it is very similar to the proof of Theorem~\ref{thm:PDexp_varying_epsilon}.

\begin{theorem}\label{thm:PDexp_varying_epsilon_conf}
For $i.i.d.$ item type sequences from a distribution $F$, the PD-exp algorithm with $\epsilon(t) = \sqrt{\frac{|\mC|}{2(t+1)}}$, $\kappa=1$, guarantees:
\[ \expct{N_F^{PD}(T)} \leq \expct{N_F^{OPT}(T)} + \sqrt{8 |\mC| T} .\]
\end{theorem}

\begin{algorithm}
\caption{{\bf PD-exp} for configuration model}
\label{alg:PDexp}
\algsetblock[Name]{Parameters}{}{0}{}
\algsetblock[Name]{Initialize}{}{0}{}
\begin{algorithmic}[1]
%\Parameters { A  sequence of strongly convex functions $f_1, f_2, \ldots$ defined on a common domain $S \subseteq \mathbb{X}$.}
%\Initialize { $\mathbf{\theta_1=0} \in \mathbb{X}$}
\For {$t=1,2,\ldots$}
\State Observe item type $Y_t$ (say, $Y_t = j$)
\State Define configuration potentials:
\begin{align*}
V_c(t-1) & := 1 - \kappa e^{ -\epsilon(t) N_c(t-1)} \\
V_\emptyset & := 0
\end{align*}
\State Place arriving item in configuration $c^*$ to create $c^* + e_j$, where:
\[ c^* = \argmin_{c: N_c(t-1)>0} V_{c +e_j}(t-1) - V_{c}(t-1) \]
\EndFor
\end{algorithmic}
\end{algorithm}

\paragraph{Running time : } For 1-dimensional packing in bins of size $B$, the possible number of configurations is given by the partition number of $B$ which grows asymptotically as $\tilde{\mO}\left( e^{\pi \sqrt{\frac{2B}{3}}} \right)$. Therefore, the configuration based Primal-Dual algorithm is not polynomial time unless the objective was minimum cost packing with cost $w_c$ for each configuration $c$ a part of the input. For $d$-dimensional vector packing with the metric of minimizing number of bins used, a level LP similar to $\mathbf{P_{1d-level}}$ can be written. The running time of Primal-Dual using the $d$-dimensional level LP is $\mO(B^{d}T)$. We do not know if this running time is necessary for $d$-dimensional vector packing.



==> tex/cornerpoint.tex <==
\section{Beyond Bounded Waste and Linear Waste: Vertex Dual distributions}
\label{sec:cornerpoint}

The \cite{courcoubetis1986necessary} characterization of distributions as Linear Waste, Perfectly Packable, and Bounded Waste seems discouraging: most distributions have Linear Waste which are bad instances for online packing. In this section we conjecture that from an algorithm design viewpoint, the opposite situation is true. We  provide evidence that most distributions are in fact easy to pack; the Primal-Dual Algorithm~\ref{alg:PDexp} can pack them with $\mO(\log^{1+\beta} T)$ regret (for any $\beta>0$) compared to the optimal in hindsight. Further, this $\mO(\log^{1+\beta} T)$ regret result is robust to non-stationary input sequences under the constraint that each distribution in the sequence is at most a small perturbation from a base distribution.

To make a more formal conjecture, it is more convenient to use the configuration model from Section~\ref{sec:PDconf}. We begin with the dual for problem $\mathbf{P_{conf}}$ by introducing dual variables $\alpha_c$ for the first set of non-negativity constraints, and $z_j$ for the second set of mass conservation constraints:
\begin{align*}
 & \max_{ \{z_j\}_{[J]} , \{\alpha_c\}_{\mC} } \sum_{j \in [J]} p_j z_j & \mathbf{(D_{conf})}\\
\mbox{subject to } \quad &  \forall c \in \mC \ : \ \alpha_c \geq 0 \\
 & \forall c \in \mC \ : \ \sum_{j} z_j x_{cj}  = 1 - \alpha_c
\end{align*}
which we further simplify to:
\begin{align*}
 & \max \sum_{j \in [J]} p_j z_j & \mathbf{(D'_{conf})}\\
\mbox{subject to } \quad & \forall c \in \mC \ : \ \sum_{j} z_j x_{cj}  \leq 1
\end{align*}
The $|\mC|$ constraints define a polytope of feasibility for $\{z_j\}$, call it $\mZ$. Note that $\mZ$ is a function of the support of the distribution $U_F$ and the set of feasible configurations $\mC$. Let $z^*(F) \in \mZ$ be a maximizer of $\mathbf{D'_{conf}}$ for distribution $F$.

\begin{definition}[Vertex-Dual distribution] A distribution $F$ is called a vertex dual (VD) distribution if $z^*(F)$ is unique. Note that $z^*(F)$ must then necessarily be an extreme point of the polytope $\mZ$.
\end{definition}

VD distributions are universal in the sense that for a given support $U$ of item types, any perturbation of a distribution (with no atoms in the perturbing noise) gives a VD distribution with probability 1. Further, they are robust in the sense that if we start with a VD distribution, then a small enough perturbation keeps the distribution VD with the same vertex $z^*$. 

For an extreme point $z^\dagger$ of $\mZ$,  let $\mathcal{P}(z^\dagger)$ denote the set of all VD distributions corresponding to $z^\dagger$:
\[ \mathcal{P}(z^\dagger) = \{ F |  z^*(F) = z^\dagger \mbox{ is unique}\}. \]

Let $\mathcal{P}(z^{\dagger},\delta)$ denote the set of all VD distributions whose $\delta$ ball is contained in $\mathcal{P}(z^\dagger)$:
\[ \mathcal{P}(z^\dagger, \delta) = \{ F | F' \in \mathcal{P}(z^\dagger) \ \forall\  ||F'-F||_{\infty}\leq \delta \}. \]

We next present our conjecture which states that VD distributions are in fact easy to pack online.

\begin{conjecture}[$\mO(\log^{1+\beta} T)$ regret for VD distributions]
\label{conj:cornerpoint}
Let the packing instance $Y = \{ Y_1, \ldots, Y_T\}$ be generated by sampling $Y_t$ from $F_t$ independently, and where each $F_t \in \mathcal{P}(z^\dagger, \delta)$ for some $\delta> 0$, and some extreme point $z^\dagger$ of $\mZ$. Then, applying the PD-exp Algorithm~\ref{alg:PDexp} with $\epsilon(t) = \Theta\left( \frac{1}{\log^{1+\beta} t} \right)$ for any $\beta > 0$,
\[ \expct{N^{PD}(T) - N^{OPT}(T)} \leq \mO(\log^{1+\beta} T). \]
\end{conjecture}
%Conjecture~\ref{conj:cornerpoint} is complementary to Theorem~\ref{thm:adversarial_smoothed} : If for an $L$-bounded fractional partition $\pi$, the smoothed distributions $\{ \hat{F}_{\pi,1}, \hat{F}_{\pi,2}, \ldots \}$ satisfy the conditions given above, then we conjecture that an appropriate choice of $\epsilon(t)$ in PD-exp algorithm should achieve a regret that grows polylogarithmically in $T$, and at most polynomially in $L$.


In Figure~\ref{fig:PD_CP}, we provide experimental evidence for Conjecture~\ref{conj:cornerpoint}. The figure shows three single simulation run of a non-stationary online packing instance with $T=2\times 10^5$, $T=2\times 10^6$, and $2\times 10^7$. The bin size is $B=9$, and the support of the distributions is $U=\{2,3\}$ The distribution at time $t$ is given by a convex combination of $F_L = \{p_2 = \frac{43}{48}, p_3 = \frac{5}{48}\}$ and $F_U = \{p_2 = \frac{37}{48}, p_3 = \frac{11}{48}\}$. The weights are given by a sinusoidal function whose period was chosen to accommodate 10 full cycles of the sin function. All the distributions thus used are VD distributions associated with the unique dual $z = \{ z_2 = \frac{1}{4}, z_3 = \frac{1}{4}\}$. We set $\epsilon(t) = \frac{1}{\log^{1.5} (t+10)}$ in Algorithm~\ref{alg:PDexp}. The waste of PD-exp is remarkably close to the offline optimal and, as shown in the second plot, the regret appears to grow polynomially in $\log t$.

\begin{figure}[ht]
\hspace{-0.1in}
\begin{minipage}{7.2in}
\begin{minipage}{2.35in}
\includegraphics[width=2.25in]{Waste_cos_CP_2E5}
\subfigure[$T=2\times 10^5$]{\includegraphics[width=2.3in]{Regret_cos_CP_2E5}}
\end{minipage}
\begin{minipage}{2.35in}
\includegraphics[width=2.25in]{Waste_cos_CP_2E6} \\
\subfigure[$T=2\times 10^6$]{\includegraphics[width=2.3in]{Regret_cos_CP_2E6}}
\end{minipage}
\begin{minipage}{2.35in}
\includegraphics[width=2.25in]{Waste_cos_CP_2E7}
\subfigure[$T=2\times 10^7$]{\includegraphics[width=2.3in]{Regret_cos_CP_2E7}}
\end{minipage}
%\subfigure[Waste ($W^{PD}(t), W^{OPT}(t)$)]{\includegraphics[width=3.5in]{Waste_sin_CP_2}}
%\hspace{-0.1in}
%\subfigure[Regret ($W^{PD}(t)-W^{OPT}(t)$)]{\includegraphics[width=3.5in]{Regret_sin_CP_logscale_2}}
\end{minipage}
\caption{Simulation results showing the performance of PD-exp on a non-stationary arrival sequence where the distributions $F_t$ are all VD distribution with a common unique dual. The arrival distributions were generated by taking convex combination of two distributions, with weights given by a sinusoidal function. The period of the sin function was chosen to accommodate 10 cycles in the total number of arrivals simulated. The top subplots show waste of the PD-exp algorithm and the waste of the optimal offline (which can repack items) vs. number of arrivals. The bottom subplot shows the regret vs. time ($\log$-scale). The growth rate of regret in each subplot, as well the final values across the three subplots suggest that the regret is growing as $\mO(\polylog t)$.
}
\label{fig:PD_CP}
\end{figure}

\paragraph{Intuition for Conjecture~\ref{conj:cornerpoint}}: First observe that for a VD distribution, given the unique optimal dual solution $z^*$, one optimal solution for dual variables for the non-negativity constraints $n_c \geq 0$ is given by: $\alpha^*_c = 1 - \sum_j z_j^* x_{cj}$. By complementary slackness, $\alpha^*_c > 0$ implies $n_c=0$ in the optimal solution. Call the configurations $c$ with $\alpha^*_c > 0$ non-basic configurations, and the rest basic configurations. To prove the conjecture, it would suffice if we prove that for any non-basic configurations $c$, the number of bins in configuration $c$ at the end of the packing horizon is small: $N_c(T) = \mO(\log^{1+\beta} T)$. 
 We now use the observation that the Primal-Dual algorithm is essentially a stochastic gradient ascent algorithm for maximizing the dual function $q(\alpha)$ of which $\alpha^*$ is a maximizer. %(analogous to \eqref{eqn:dualfn1}), of which $\alpha^*$ is a maximizer.
 Further, for all distributions within $\mathcal{P}(z,\delta)$, the optimal solution is the same. Now we would be done if the following two conditions were met: ($i$) $\alpha^*$ is unique, and ($ii$) the subgradient of function $q(\alpha)$ is bounded away from 0 everywhere. This would imply that $\expct{e^{ \frac{1}{\epsilon} ||V(t)-v^*||}}=\mO(1)$ where $v^*=1-\alpha^*$ and $V(t)$ are as in Algorithm~\ref{alg:PDexp_level}, and therefore, $\prob{||V(t)-v^*|| \geq \frac{K}{\log^\beta T} } = o(1/T)$ (for some constant $K>0$). A similar idea has been used by \cite{huang2011delay} in a queueing control setting. %For example, in certain queuing contexts where these conditions are true, Lyapunov function based policies yield $(1+\epsilon)$ competive control strategies with $\mO\left(\log^2 \frac{1}{\epsilon} \right)$ delay (\cite{huang2011delay}). 

However, in our case $\alpha^*$ is not unique, and therefore $q(\alpha)$ does not possess subgradients bounded away from 0 everywhere. This is the challenge in proving the Conjecture. 
Fortunately, an analysis along similar lines as that of BW distributions in \cite{SumOfSquares_JACM_CsirikJKOSW06} seems possible -- we further classify the non-basic configurations into \emph{live configurations} (those to which items can be added to reach a basic configuration), and \emph{dead-end configurations} (all others). We now observe that $\alpha^*_c$ is unique for all live configurations $c$, and $\alpha^*_c$ for dead-end configurations lie in a low dimensional subspace. The subgradient of the dual function $q(\alpha)$ are bounded away from 0 when restricted to deviations from these subspaces.

Conjecture~\ref{conj:cornerpoint} is reminiscent of recent results on network revenue management where uniqueness of the dual solution to the offline LP is used to prove that resolving heuristics with probabilistic acceptance rules give $\mO(1)$ regret in the case of known demand parameters (\cite{jasin2012re}), and $\mO(\log^2 T)$ regret in the case of unknown demand parameters which are learned online (\cite{jasin2015performance}). Our conjecture suggests that in the case of unknown demand parameters, it may be possible to obtain $\mO(\log^{1+\beta} T)$ regret without any explicit learning,  even when demand is somewhat non-stationary.

%[TODO]: redo using level, move sec 6 to appendix, add bounded inventory conjecture


==> tex/cornerpoint_level.tex <==
\section{Beyond Bounded Waste and Linear Waste: Corner Point distributions}
\label{sec:cornerpoint}

The \cite{courcoubetis1986necessary} characterization of distributions as Linear Waste, Perfectly Packable, and Bounded Waste seems discouraging: most distributions have Linear Waste which are bad instances for online packing. In this section we conjecture that from an algorithm design viewpoint, the opposite situation holds. We  provide evidence that most distributions are in fact easy to pack; the Primal-Dual Algorithm~\ref{alg:PDexp} can pack them with $\mO(\log^{1+\beta} T)$ regret (for any $\beta>0$) compared to the optimal in hindsight. Further, this $\mO(\log^{1+\beta} T)$ regret result is robust to non-stationary input sequences where each distribution in the sequence is restricted to be at most a small perturbation from a base distribution.

To make a more formal conjecture, we return to the bin packing problem from Section~\ref{sec:PDbasic} and rewrite the dual problem $\mathbf{D_{conf}}$:
\begin{align*}
 & \max \sum_{j \in [J]} p_j z_j & \mathbf{(D'_{conf})}\\
\mbox{subject to } \quad & \forall c \in \mC \ : \ \sum_{j} z_j x_{cj}  \leq 1
\end{align*}
The $|\mC|$ constraints define a polytope of feasibility for $\{z_j\}$, call it $\mZ$. Note that $\mZ$ is a function of the support of the distribution $U_F$ and the set of feasible configurations $\mC$. Let $z^*(F) \in \mZ$ be a maximizer of $\mathbf{D'_{conf}}$ for distribution $F$.

\begin{definition}[Corner-Point distribution] A distribution $F$ is called a corner point (CP) distribution if $z^*(F)$ is unique. Note that $z^*(F)$ must then necessarily be an extreme point of the polytope $\mZ$.
\end{definition}

CP distributions are universal in the sense that for a given support $U$ of item types, any perturbation of a distribution (with no atoms in the perturbing noise) gives a CP distribution with probability 1. Further, they are robust in the sense that if we start with a CP distribution, then there is a small enough perturbation keeps the distribution CP with the same corner $z^*$. 

For an extreme point $z^\dagger$ of $\mZ$,  let $\mathcal{P}(z^\dagger)$ denote the set of all CP distributions corresponding to $z^\dagger$:
\[ \mathcal{P}(z^\dagger) = \{ F |  z^*(F) = z^\dagger \mbox{ is unique}\}. \]

Let $\mathcal{P}(z^{\dagger},\delta)$ denote the set of all CP distributions whose $\delta$ ball is contained in $\mathcal{P}(z^\dagger)$:
\[ \mathcal{P}(z^\dagger, \delta) = \{ F | F' \in \mathcal{P}(z^\dagger) \ \forall\  ||F'-F||_{\infty}\leq \delta \}. \]

We next present our conjecture which states that CP distributions are in fact easy to pack online.

\begin{conjecture}[$\mO(\log^{1+\beta} T)$ regret for CP distributions]
\label{conj:cornerpoint}
Let the packing instance $Y = \{ Y_1, \ldots, Y_T\}$ be generated by sampling $Y_t$ from $F_t$ independently, and where each $F_t \in \mathcal{P}(z^\dagger, \delta)$ for some $\delta> 0$, and some extreme point $z^\dagger$ of $\mZ$. Then, applying the PD-exp Algorithm~\ref{alg:PDexp} with $\epsilon(t) = \Theta\left( \frac{1}{\log^{1+\beta} t} \right)$ for any $\beta > 0$,
\[ \expct{N^{PD}(T) - N^{OPT}(T)} \leq \mO(\log^{1+\beta} T). \]
\end{conjecture}

Before we provide intuition for why we expect Conjecture~\ref{conj:cornerpoint} to be true, we provide some experimental evidence. In Figure~\ref{fig:PD_CP}, we show a single simulation run of a non-stationary online packing instance with $T=10^6$. The bin size is $B=9$, and the support of the distributions is $U=\{2,3\}$ The distribution at time $t$ is given by a convex combination of $F_L = \{p_2 = \frac{43}{48}, p_3 = \frac{5}{48}\}$ and $F_U = \{p_2 = \frac{37}{48}, p_3 = \frac{11}{48}\}$: $ F_t = \frac{F_U+F_L}{2} + \frac{F_U-F_L}{2} \cdot \sin \left( \frac{2\pi t}{100000} \right)$. All the distributions thus used are CP distributions associated with the uniqe dual $z = \{ z_2 = \frac{1}{4}, z_3 = \frac{1}{4}\}$. We set $\epsilon(t) = \frac{1}{\log^{1.2} (t+10)}$ in Algorithm~\ref{alg:PDexp}. The waste of PD-exp is remarkably close to the offline optimal and, as shown in the second plot, the regret appears to grow polynomially in $\log t$.

\begin{figure}[ht]
\hspace{-0.1in}
\begin{minipage}{7.2in}
\subfigure[Waste ($W^{PD}(t), W^{OPT}(t)$)]{\includegraphics[width=3.5in]{Waste_sin_CP_2}}
\hspace{-0.1in}
\subfigure[Regret ($W^{PD}(t)-W^{OPT}(t)$)]{\includegraphics[width=3.5in]{Regret_sin_CP_logscale_2}}
\end{minipage}
\caption{Simulation results showing the performance of PD-exp on a non-stationary arrival sequence where the distributions $F_t$ are all CP distribution with a common unique dual. The first subplot shows the waste of the PD-exp algorithm vs. the waste of the optimal offline (which can repack items). The second subplot shows the regret vs. time, and suggests that the regret is growing as $\mO(\polylog t)$.
}
\label{fig:PD_CP}
\end{figure}

\paragraph{Intuition for Conjecture~\ref{conj:cornerpoint}}: First observe that for a CP distribution, given the unique optimal dual solution $z^*$, one optimal solution for dual variables for the non-negativity constraints $n_c \geq 0$ is given by: $\alpha^*_c = 1 - \sum_j z_j^* x_{cj}$. By complementary slackness, $\alpha^*_c > 0$ implies $n_c=0$ in the optimal solution. Call the configurations $c$ with $\alpha^*_c > 0$ non-basic configurations, and the rest basic configurations. To prove the conjecture, it would suffice if we prove that $N_c(T) = \mO(\log^{1+\beta} T)$ for all non-basic configurations. 
 We now use the observation that the Primal-Dual algorithm is essentially a stochastic gradient ascent algorithm for maximizing the dual function $q(\alpha)$ (analogous to \eqref{eqn:dualfn1}), of which $\alpha^*$ is a maximizer. Further, for all distributions within $\mathcal{P}(z,\delta)$, the optimal solution is the same. Now we would be done if the following two conditions were met: ($i$) $\alpha^*$ is unique, and ($ii$) the subgradient of function $q(\alpha)$ is bounded away from 0 everywhere. %For example, in certain queuing contexts where these conditions are true, Lyapunov function based policies yield $(1+\epsilon)$ competive control strategies with $\mO\left(\log^2 \frac{1}{\epsilon} \right)$ delay (\cite{huang2011delay}). 

However, in our case $\alpha^*$ is not unique, and therefore $q(\alpha)$ does not possess subgradients bounded away from 0 everywhere. This is the challenge in proving the Conjecture. 
Fortunately, an analysis along similar lines as that of BW distributions in \cite{SumOfSquares_JACM_CsirikJKOSW06} seems possible -- we further classify the non-basic configurations into \emph{live configurations} (those to which items can be added to reach a basic configuration), and \emph{dead-end configurations} (all others). We now observe that $\alpha^*_c$ is unique for all live configurations $c$, and $\alpha^*_c$ for dead-end configurations lie in a low dimensional subspace. The subgradient of the dual function $q(\alpha)$ are bounded away from 0 when restricted to deviations from these subspaces.

[TODO]: redo using level, move sec 6 to appendix, add bounded inventory conjecture


==> tex/ecompanion.tex <==

%% Here starts the e-companion (EC)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ECSwitch

%\ECDisclaimer
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Main head for the e-companion
\ECHead{Online Convex Optimization view of Primal-Dual algorithms}

In this section we show that how the guarantees proved in Theorems~\ref{thm:PDexp_fixed_epsilon} and \ref{thm:adversarial_smoothed} can be derived via the framework of Online Convex Optimization.

Main OCO setting: predict $\theta_t$, receive loss function $f_t$, goal to minimize regret:
\[ \mathcal{R}(T) = \sum_{t=1}^T \inn{f_t}{\theta_t} - \min_{\theta \in \Theta} \sum_{t=1}^T \inn{f_t}{\theta} \]

Need to define:
\begin{enumerate}
\item Space $\Theta$
\item A norm $||\cdot||$ on $\Theta$
\item A distance generating function $\omega(\cdot)$ on $\Theta$ so that it is $1$-strongly convex with respect to $||\cdot||$. That is: 
\[ \omega(y) \geq  \omega(x) + \inn{\omega'(x)}{y-x} + \frac{1}{2} ||y-x||^2\]
or equivalently,
\[ \inn{\omega'(y)-\omega'(x)}{y-x} \geq ||y-x||^2\]
\item Bregman distance of $y$ from $x$:
\[ V_x(y) = \omega(y) - \omega(x) - \inn{\omega'(x)}{y-x}\]
Strong convexity of $\omega$ implies $V_x(y) \geq \frac{1}{2}||y-x||^2$.
\item Define $\omega$-radius of $\Theta$:
\[ \frac{1}{2}D^2  = \max_{\theta \in \Theta} \omega(\theta) - \min_{\theta \in \Theta} \omega(\theta) \]
\item Boundedness of gradients:
\[ \sup_{\theta \in \Theta} ||f_t(\theta)||_* \leq G\]
\end{enumerate}

\begin{theorem}[OCO Regret gives the bound stated in the theorem. guarantee]
The proximal descent algorithm:
\[ \theta_{t+1} = \argmin_{\theta} \epsilon \inn{ \sum_{s=1}^t f_s}{\theta}  + \omega(\theta)  \]
or equivalently:
\[\theta_{t+1} = \argmin_{\theta} \epsilon \inn{f_t}{\theta} + V_{\theta_t}(\theta) \]
with $\epsilon = \frac{D}{G\sqrt{T}}$
gives:
\[ \mathcal{R}(T) \leq DG \sqrt{T} \]
\end{theorem}
\proof{Proof:}
The basic Mirror Descent inequality says:
\[ \inn{\epsilon f_t}{\theta_t - z} \leq V_{\theta_t}(z) - V_{\theta_{t+1}}(z) + \underbrace{ \inn{\epsilon f_t}{\theta_t - \theta_{t+1}} - V_{\theta_t}(\theta_{t+1})}_{ \leq ||\epsilon f_t||_* ||\theta_t - \theta_{t+1}|| - \frac{1}{2}||\theta_t-\theta_{t+1}||^2 \leq \frac{1}{2}||\epsilon f_t||_*^2}  \]
For the inequality in underbrace: $ab - \frac{a^2}{2} \leq \frac{b^2}{2}$.
Therefore:
\[ f(\theta_t) - f(z) \leq  \inn{f_t}{\theta_t - z} \leq \frac{V_{\theta_t}(z) - V_{\theta_{t+1}}(z)}{\epsilon} + \frac{\epsilon}{2} ||f_t||_*^2  \]
A telescoping sum gives:
\[ \mathcal{R}(T) \doteq \sum_{t=1}^T f(\theta_t) - T \min_{z} f(z) \leq \frac{D^2}{2\epsilon} + \frac{\epsilon G^2 }{2} T \]
which after setting $\epsilon = \frac{D}{G\sqrt{T}}$ gives the bound stated in the theorem.
\endproof \Halmos

Applied to our setting:
\begin{enumerate}
\item The space $\Theta = [0, 1]^{|\mC|}$ (the space of configuration duals)
\item The distance generating function will be entropy:
\[ \omega(\alpha) = \sum_c \alpha_c (\log \alpha_c - 1)\]
with the Bregman distance function:
\[ V_{x}(y) = \sum_c y_c \log y_c - \sum_c y_c \log x_c - \sum_c (y_c-x_c)\]
and 
\[ \frac{\partial V_{x}(y)}{\partial y} = \{  \log y_c - \log x_c \}  \]
\item The norm will be $||\cdot|| = \ell_2$ and dual norm $||\cdot||_* = \ell_{2}$
\item The function we are \emph{minimizing} is the negative dual function:
\[ f(\alpha)  = - q(\alpha) = - \sum_j p_j \sum_c (1-\alpha_c) a^*_{cj}\]
where $a^*_{j} = \argmin_{a \in A_j} \sum_c (1-\alpha_c)a_j$, and 
\[ A_j = \{ u_{c} | x_{cj} > 0 \} \union \{ u_c - u_{c-e_j} | x_{cj}>0, x\neq e_j \}\]
Note that the first set of actions allows us to open fresh bins and mark then as configuration $c$. As we show soon, if $N_{c-e_j} = 0$, this action is always preferred over $(u_c - u_{c-e_j}) $ and therefore we do not create negative bins. In other words, the primal solution we will obtain will always be feasible.
\item The gradient $f_t = a_{Y_t}$, where $Y_t$ is the random type of the arriving item, and $a_{Y_t}$ is the placement action taken based on $\theta_t = \alpha_t$.
\end{enumerate}

\section{Proof of Theorem \ref{thm:PDexp_fixed_epsilon}}
\begin{repeattheorem}[Theorem~\ref{thm:PDexp_fixed_epsilon}]
For the PD-exp algorithm with $\epsilon(t) = \sqrt{\frac{|\mC|}{T}}$, $\kappa=1$, and $T>|\mC|$,
\[ \expct{N_F^{PD}(T)} \leq \expct{N_F^{OPT}(T)} + \sqrt{4 |\mC|T } .\]
\end{repeattheorem}
\proof{Proof:}
{\bf Step 1: OCO guarantee} \\
\begin{align*}
\mathcal{R}(T) &= \sum_{t=1}^{T} \inn{a_t}{\alpha_t} - \min_{\alpha \in \Theta} \sum_{t=1}^T \inn{a_t}{\alpha} \\
&= \sum_{t=1}^{T} \inn{a_t}{\alpha_t} - \min_{\alpha \in \Theta} \inn{N(T)}{\alpha} \\
& \leq DG\sqrt{T}
\end{align*}
Note that $\Theta = [0,1]^{|\mC|}$ and as we argued, $N(t) \geq 0$, therefore $\min_{\alpha} \inn{N(T)}{\alpha} = 0$. For the entropy function,
\[ \omega(\alpha) = \sum_c \alpha_c \left( \log \alpha_c - 1 \right) \]
and therefore, $D = \sqrt{2 |\mC|}$. The dual norm is $||\cdot||_{*}=||\cdot||_2$ , and therefore, $G=\sqrt{2}$. This gives:
\begin{align}
\sum_{t=1}^T \inn{a_t}{\alpha_t} \leq \sqrt{4|\mC|T}
\end{align}

{\bf Step 2: Primal guarantee} \\
Let $a^*_t$ be the offline optimal primal action, and $a_t$ be the action taken by the algorithm
\begin{align*}
\inn{1-\alpha_t}{a_t} \leq \inn{1-\alpha_t}{a^*_t} \leq \max_{\alpha} \inn{1-\alpha}{a^*_t} = OPT_t
\end{align*}
Therefore,
\begin{align}
COST_T &=  \sum_{t=1}^{T} \inn{1}{a_t} \leq \sum_t OPT_t + \inn{\alpha_t}{a_t} \leq \sum_{t} OPT_t + \sqrt{4|\mC|T} 
\end{align}

\Halmos \endproof


Remarks: (1) the OCO regret guarantee gives us weak duality gap {\bf(?)}.  (2) 


\begin{lemma} The entropy function $\omega(x) = \sum_{i\in [d]} x_i (\log x_i - 1)$ is $1$-strongly convex with respect to $\ell_2$ norm in $[0,1]^d$.
\end{lemma}
\proof{Proof:} It suffices to prove:
\[ \inn{w'(x) - w'(y)}{x-y} \geq ||x-y||_2^2 \]
The LHS is:
\[ \sum_i (\log x_i - \log y_i )(x_i - y_i) \]
The RHS is 
\[ \sum_{i} (x_i-y_i)^2 \]
Now we will show:
\[ (\log a - \log b) (a-b) \geq (a-b)^2 \]
or,
\[ (a-b) \left[ (\log a - a) - (\log b - b) \right] \geq 0\]
or that $g(x) = \log x - x$ is increasing in $x \in [0,1]$. We have $g'(x) = \frac{1}{x}-1 \geq 0$ when $x\leq 1$.
\Halmos \endproof

\section{Proof of Theorem~\ref{thm:adversarial_smoothed}}
\begin{repeattheorem}
Consider the adversarial arrival model described above with a packing horizon of $T$ items, and an arbitrary conditioning time $t$. 
%For a given window size $L$, define the \emph{$L$-smoothed arrival distribution} at time $k$ conditioned on $\mathcal{F}_t$ as:
%\[ \hat{F}_{L,k|t} \doteq  \expct{ \left. \frac{1}{L} \sum_{m=k}^{k+L-1} F_m  \right| \mathcal{F}_t} \]
%Denote the optimal bin-rate of the bin packing LP for $\hat{F}_{L,k|t}$ by $\hat{b}_{L,k|t}$. For succinctness, $\hat{b}_{L,k} \doteq \hat{b}_{L,k|0}$.
Let $\epsilon$ and $\kappa$ denote the parameters of the penalized-Lagrangian function in Algorithm~\ref{alg:PDexp}. 

If $L, \epsilon, \kappa, |\mC|$ satisfy: $\epsilon L < 1$, and $L \leq \frac{1}{\epsilon} \log \frac{\kappa |\mC|}{|\mC|-1}$, then for all $\pi \in \Pi(L,T)$:
\[ \expct{ N^{PD}(T) | \mathcal{F}_t } \leq \sum_{k=1}^T \hat{b}_{\pi,k|t} +  T \kappa \epsilon \left( \frac{2L+3}{4} \right) + \frac{|\mC| \kappa }{\epsilon} . \]
\end{repeattheorem}
\proof{Proof:}
{\bf Step 1: OCO guarantee} \\
This step is identical to the previous proof, and gives:
\[ \sum_{t=1}^T \inn{\alpha_t}{a_t} \leq \frac{|\mC|}{\epsilon} + \epsilon G T .\]

{\bf Step 2: Primal Guarantee} \\
The analysis begins with bounding $\expct{ \sum_{s=1}^T \inn{1-\alpha_s}{a_s} | \F_t} $. Note that $a_t, \alpha_t$ are random variables, adapted to $\{ \F_t \}$. 

\begin{align*}
\expct{ \sum_{s=1}^T \inn{1-\alpha_s}{a_s} | \F_t} &= \expct{\sum_{k=1}^T \sum_{s=1}^T q_k(s) \inn{1-\alpha_s}{a_s} | \F_t} \\
&= \sum_k \expct{ \sum_{s=1}^T q_k(s) \inn{1-\alpha_s}{a_s} | \F_t } 
\end{align*}
Let us focus on the $k$th term above. Let $\hat{a}_k$ be the optimal action for the $k$th smoothed distribution, and let $\hat{a}^j_k$ be the component of the action corresponding to item type $j$ (that is, $\hat{a}_k = \sum_{j} \hat{p}_j \hat{a}^j_k$ where $\hat{p}_j$ is the probability of item $j$ under the conditional smoothed distribution $\hat{F}_k | \F_t$. Let $\hat{a}_{k,s} = \sum_{j} p_j(s) \hat{a}^j_k$ be the projection of the actions $\{ \hat{a}^j_k \}_{j=1}^J$ to the distribution $F_s$ at time $s$.
\begin{align*}
\expct{ \sum_{s=1}^T q_k(s) \inn{1-\alpha_s}{a_s} | \F_t } & \leq \expct{ \sum_{s=1}^T q_k(s) \inn{1-\alpha_s}{\hat{a}_{k,s}} | \F_t } \\
&= \expct{ \sum_{s=1}^T q_k(s) \inn{1-\alpha_{\ell_k}}{a_{s}} | \F_t }  + \expct{\sum_{s=1}^T \inn{ \alpha_{\ell_k}-\alpha_s }{q_k(s) \hat{a}_{k,s} } | \F_t } \\
&= \expct{ \max_{\alpha}\sum_{s=1}^T \inn{1-\alpha}{\hat{a}_{k}} | \F_t }  + \expct{\sum_{s=1}^T q_k(s) || \alpha_{\ell_k}-\alpha_s || \cdot ||\hat{a}_{k,s} ||_* | \F_t } \\
&= \hat{b}_{k,t} + \sqrt{2} \expct{\sum_{s} q_k(s) ||\alpha_{\ell_k} -\alpha_s||  | \F_t } \\
\intertext{and observing that $||\alpha_{s+1}-\alpha_s|| \leq 2 \epsilon \sqrt{2} $,}
&= \hat{b}_{\pi, k|t} + 4 \epsilon L 
\end{align*}

Combining:
\begin{align*}
\expct{N^{PD}(T)| \F_t} &= \expct{ \sum_{s=1}^T \inn{1}{a_s} | \F_t} \\
& = \expct{ \sum_{s=1}^T \inn{1-\alpha_s}{a_s} | \F_t} +  \expct{ \sum_{s=1}^T \inn{\alpha_s}{a_s} | \F_t} \\
& \leq \sum_k \hat{b}_{\pi, k|t} + 4\epsilon L T + \frac{|\mC|}{\epsilon} + \sqrt{2}\epsilon T \\
& = \sum_k \hat{b}_{\pi, k|t} + \epsilon (4L+\sqrt{2}) T + \frac{|\mC|}{\epsilon} \\
\end{align*}
\endproof \Halmos

\begin{lemma}
Consider the projected Mirror Descent step:
\[ \alpha_{t+1} = \argmin_{\alpha \in \Omega} \epsilon \inn{\alpha}{g_t} + V_{\alpha_t}(\alpha). \]
Then,
\[ ||\alpha_{t+1} - \alpha_t|| \leq 2 \epsilon ||g_t||_* .\]
\end{lemma}
\proof{Proof}
We use the fact that 1-strong convexit of the distance generating function corresponding to $V()$ implies $V_{x}(y) \geq \frac{1}{2}||x-y||^2$. Then:
\begin{align*}
\epsilon \inn{\alpha_{t+1}}{g_t} + \frac{1}{2}||\alpha_t-\alpha_{t+1}||^2 &\leq \epsilon \inn{\alpha_{t+1}}{g_t} + V_{\alpha_t}(\alpha_{t+1}) \\
& \leq \epsilon \inn{\alpha_t}{g_t} + V_{\alpha_t}(\alpha_t) \\
&= \epsilon \inn{\alpha_t}{g_t} 
\end{align*}
Therefore:
\[ \frac{1}{2} ||\alpha_t - \alpha_{t+1}||^2 \leq \epsilon \inn{\alpha_t - \alpha_{t+1}}{g_t}  \leq \epsilon ||\alpha_t - \alpha_{t+1}|| \cdot ||g_t||_*\]
or,
\[  ||\alpha_t - \alpha_{t+1}|| \leq 2 \epsilon ||g_t||_*. \]
\endproof \Halmos


==> tex/extensions.tex <==
\section{Extensions} \label{sec:extensions}

\subsection{Continuous item size distributions}

If the distribution is integer + continuous with bounded density then can pack with regret $\mathcal{O}(T^{2/3})$.

\subsection{Packing with partial information}

If know basic feasible configurations (say $J$), then can pack with regret $\sqrt{M|J|T}$ where $M$ is the maximum number of items in any configuration. 
{\bf Algorithm 1: } Use the objective function 
\[ \sum_{c \in J} \frac{1}{\eta} \log \left( e^{\eta \frac{V_{c,j}}{x_{c,j}}} \right)\]
to assign items to a configuration. 

{\bf Algorithm 2: } Use SS between non-basic feasible configurations. For 1-D packing, this should outperform Algorithm 1. For d-dimensional packing, this may be better if the 

\begin{proposition}
For corner point distributions, Algorithm 2 gets $\mO(\log T)$ additive suboptimality gap.
\end{proposition}
\begin{proof}
Should be an easy extension of original SS proof?
\end{proof}


==> tex/nonstationary_old_21Mar2019.tex <==
\section{Analysis for non-$i.i.d.$ input sequences}
\label{sec:nonstationary}

As we mentioned in the introduction, one of our motivations behind designing distribution-oblivious online packing algorithms is that we hope they will be robust to non-stationary input sequences.
Our goal in this Section is not to devise new algorithms for non-stationary input models, but show that Algorithm~\ref{alg:PDexp_level} by virtue of being distribution oblivious has good performance under non-stationary input.
 However, unlike performance guarantees proved for \emph{i.i.d.} input against the offline optimal $\expct{N^{\OPT}_{F,T}}$ in Theorem~\ref{thm:PDexp_fixed_epsilon}, the offline optimal turns out to be an unrealistic benchmark in the non-stationary case. Instead, our theorems take the form of a family of upper bounds on $\expct{N^{\PDexp}_T}$ all of which hold simultaneously. The tightest upper bound within this family will depend on the specific instance, and we will not pursue this step in full generality here. %To prove these bounds, we will need a few new ideas which we explain in due course below.

To keep the exposition simple, in this section we will prove guarantees of the $\PDexp$ heuristic for two specific models of non-{\it i.i.d.} sequences:

\begin{enumerate}
\item Independent but not identically distributed: An arbitrary sequence of distributions $\{F_1, F_2, \ldots, F_T\}$  is decided by an adversary (unknown to the online algorithm). Nature then generates the sequence $Y=\{Y_1, \ldots, Y_T\}$ by sampling $Y_t$ from distribution $F_t$ independent of other $Y_s$'s. (Section~\ref{sec:i-ni-d})
\item Identically distributed but not independent: In this case we assume that first Nature generates a sequence $\{Y_1,Y_2,\ldots, Y_T \}$ by {\it i.i.d.} sampling from a distribution $F$. The adversary is then allowed to ``locally perturb''  the sequence before it is presented sequentially to the online packing algorithm. (Section~\ref{sec:ni-i-d})
\end{enumerate}

\subsection{Independent but not identically distributed model}
\label{sec:i-ni-d}

\textbf{Model: } An arbitrary sequence of distributions $\mathbf{F}= \{ F_1, F_2, \ldots, F_T \}$ is generated, possibly adversarially. Given $\mathbf{F}$, the sequence of item sizes $\mathbf{Y} = \{Y_1, Y_2, \ldots, Y_T\}$ is generated by sampling $Y_t$ from $F_t$ independent of $Y_{s}$ ($s \neq t$).

\noindent {\bf A naive analysis : } If we naively extend the proof of Theorem~\ref{thm:PDexp_fixed_epsilon}, we get that the number of bins used by $\PDexp$ algorithm is bounded by:
\begin{align}
\label{eqn:naivenonstationary}
\expct{N^{\PDexp}_{\{F_t\},T}} &\leq \sum_{t=1}^T b(F_t) + \sqrt{4BT}. 
\end{align}

The following example illustrates that the above bound on the performance of $\PDexp$ can be too pessimistic.

\noindent \textbf{Example:} Consider a packing instance with $B=9, J=3$. The sequence of distributions is $\mathbf{F} = \{ 
 \underbrace{G_2, \ldots , G_2}_{3 T^{1/4}},
 \underbrace{G_3, \ldots, G_3}_{T^{1/4}} ,
 \ldots,
 \underbrace{G_{2}, \ldots , G_{2}}_{3 T^{1/4}}, 
 \underbrace{G_{3}, \ldots , G_{3}}_{T^{1/4}}
 \}$ where $G_2 := \{ p_2 = 1\}$ and $G_3 := \{p_3=1\}$ are deterministic distributions. That is, the sequence $\mathbf{Y}$ has $T^{3/4}/4$ phases of length $4T^{1/4}$ each. Within each phase, the first $3T^{1/4}$ items are of size $2$ and the last $T^{1/4}$ items are of size $3$. 


%Recall that $b(F)$ denotes the optimal value of $\mathbf{P_{1d-level}}$ giving the number of bins used per item in the optimal fractional packing.
We have $b(G_2)= 1/4$ and $b(G_3) = 1/3$. Therefore, $ \bar{b}(\mathbf{F}) := \frac{1}{T}\sum_{t=1}^T b(F_t) = \frac{13}{48} \approx 0.271$. However, for the \emph{average} distribution $\bar{\bF} := \frac{1}{T} \sum_{t=1}^T F_t = ( p_2 = 3/4, p_3 = 1/4 )$, $b(\bar{\mathbf{F}}) = 1/4 = 0.25$. Therefore we should expect the entire instance to be packed with sublinear waste, even though the distributions for a constant fraction of time steps are Linear Waste distributions (i.e., $G_2$). We will prove that for this instance $\PDexp$ indeed gives this desired result. We should also point out that a naive learning based algorithm which uses change point detection, re-solves the LP for optimal packing, and then packs using the optimal solution of the LP, will incur linear waste.

\noindent {\bf Towards a more sophisticated analysis : } The reason the naive analysis yields a somewhat bad result is apparent from the proof of Theorem~\ref{thm:PDexp_fixed_epsilon}, where the change in Lagrangian at a given time $t$ is upper bounded by the change in Lagrangian due to a probabilistic policy $A_{F_t}$ which depends on the distribution from which the item at time $t$ is generated. Hence the term $b(F_t)$ in the upper bound given in \eqref{eqn:naivenonstationary}. To get a tighter bound it is not sufficient to bound the change in Lagrangian at a {\it deterministic time} $t$; we need to define random times. For example, consider the random time $S_1$ which has a uniform distribution on $[4 T^{1/4}]$. The distribution of the arriving item at the random time $S_1$ is $F_{S_1} = ( p_2 = 3/4, p_3=1/4 )$ with $b(F_{S_1})=0.25 = b(\bar{\mathbf{F}}) < \bar{b}(\mathbf{F})$. Our goal is to bound the change in Lagrangian from time $t=0$ to $t=T$ via such random times whose distributions are smeared out enough so that the average item size distribution at such random times $S_t$ are ``nicer'' -- that is, have small $b(F_{S_t})$. Since $b(F)$ is a convex function of $F$ (Proposition~\ref{prop:flowLP_props}), the larger the support of these random times, lower the $b(F_{S_t})$. But as our main theorem (Theorem~\ref{thm:adversarial_smoothed}) shows, there is a trade-off that must be optimized.

\noindent {\bf Analysis:} As we mentioned, the crux of analysis is to calculate the change in Lagrangian at a random time so that the ``smoothed'' item size distribution at this random time has a smaller objective function value than at a deterministic time. Therefore, we need to define a collection of $T$ distributions for $T$ random times $\{S_1, \ldots, S_T\}$ which must satisfy the condition that the total change in Lagrangian over $\{1,\ldots, T\}$ equals the total change in Lagrangian over $\{S_1, \ldots, S_T\}$. It turns out we do not need the joint distributions of these $T$ random times but only their marginals. Towards this, we begin by defining what we call \emph{$L$-bounded fractional partition} of the time horizon $[T]$.

\begin{definition}[$L$-bounded fractional partition] A collection $\pi = \{ q_1, q_2, \ldots, q_T \}$ of $T$ probability measures, each with support on $[T]$ is called an $L$-bounded fractional partition of the time horizon $\{1,2,\ldots, T\}$ if it satisfies:
\begin{enumerate}
\item {\bf Bounded $L$-Support:} For all $u \in [T]$, $\max \{u : q_t(u)>0 \}-\min\{u : q_t(u)>0\} \leq L-1 $
\item {\bf Unit coverage:} For all $u \in [T]: \ \sum_t q_t(u) = 1$. Equivalently, the matrix $Q = [Q_{ij}] = [q_i(j)]$ is doubly stochastic.
\end{enumerate}
Let $\ell_t = \min\{u: q_t(u) > 0\}$ denote the earliest time $u$ in the support of $t$th window, and without loss of generality assume the windows are indexed so that $\ell_t$ is non-decreasing in $t$. Let $\Pi(L,T)$ denote the set of all $L$-bounded fractional partitions of $[T]$.
\end{definition}

See Figure~\ref{fig:partition_example} for an illustration. In words, window $t$ is defined by a probability measure $q_t$ on $\{1,\ldots, T\}$ which gives the distribution of random time $S_t$ (which we will interchangeably also call the $t$th smoothing window). The $L$-boundedness condition says that no smoothing window can have support on time instants more than $L$ apart, and the distribution for each time instant $t$ is completely partitioned across the $T$ windows in $\pi$. We will assume that the partition is deterministic, that is independent of $\{Y_1,\ldots, Y_T\}$. Indeed, the simplest example is \emph{blocked partitioning} where $q_{iL+1} = q_{iL+2} = \cdots = q_{(i+1)L} = \mbox{Unif}\{iL+1,iL+2, \ldots, (i+1)L\}$, $i=1,\ldots, \frac{T}{L}$.

\begin{figure}[ht!]
\centering
\includegraphics[width=5.5in]{partition}
\caption{An illustration of $L$-bounded fractional partitions of $[T]=\{1,2,\ldots,T\}$.}
\label{fig:partition_example}
\end{figure}

\begin{definition} Given an $L$-bounded fractional partition $\pi = \{q_t\}_{t\in [T]}$, the $t$th \emph{smoothed item size distribution} is defined to be:
\begin{align}
\hat{F}_{\pi, t} := \sum_{u=1}^T q_t(u) F_t 
\end{align}
Denote the optimal bin rate of $\mathbf{P_{1d-level}}$ with distribution $\hat{F}_{\pi, t }$ by $\hat{b}_{\pi, t} := b(\hat{F}_{\pi,t})$.
\end{definition}

We are now ready to state our main result of this section.

\begin{theorem} \label{thm:adversarial_smoothed}
Consider the independent but non-identical arrival model described above with a packing horizon of $T$ items. 
%For a given window size $L$, define the \emph{$L$-smoothed arrival distribution} at time $k$ conditioned on $\mathcal{F}_t$ as:
%\[ \hat{F}_{L,k|t} \doteq  \expct{ \left. \frac{1}{L} \sum_{m=k}^{k+L-1} F_m  \right| \mathcal{F}_t} \]
%Denote the optimal bin-rate of the bin packing LP for $\hat{F}_{L,k|t}$ by $\hat{b}_{L,k|t}$. For succinctness, $\hat{b}_{L,k} \doteq \hat{b}_{L,k|0}$.
Let $\epsilon_t = \epsilon$ and $\kappa$ denote the parameters of the penalized-Lagrangian function in Algorithm~\ref{alg:PDexp_level}. 

If $L, \epsilon, \kappa, B$ satisfy: $\epsilon L < 1$, and $L \leq \frac{1}{\epsilon} \log \frac{\kappa B}{B-1}$, then for all $L$-bounded fractional partitions $\pi \in \Pi(L,T)$, the expected number of bins used in packing the sequence $\mathbf{Y}=\{Y_1,\ldots, Y_T\}$ by Algorithm~\ref{alg:PDexp_level} is upper bounded by
\[ \expct{ N^{\PDexp}_T } \leq \sum_{t=1}^T \hat{b}_{\pi,t} +  T \kappa \epsilon \left( L + \frac{3}{2} \right) + \frac{B \kappa }{\epsilon} . \]
As a corollary, setting $\kappa=3$, for $\epsilon L < 1$.
\[ \expct{ N^{\PDexp}_T } \leq \min_{\pi \in \Pi(L,T)} \sum_{t=1}^T \hat{b}_{\pi,t} +  9 T \epsilon L + \frac{3B}{\epsilon} . \]
\end{theorem}



The proof of Theorem~\ref{thm:adversarial_smoothed} appears in Appendix~\ref{sec:proofs}.
The main idea in a nutshell, again, is to calculate the change in the Lagrangian over a random time distributed according to the measure $q_t$. We can view this as calculating the change in Lagrangian in a single time step with item size distribution being the smoothed distribution $\hat{F}_{\pi,t}$ but where the packing seen by the arriving job is random and potentially correlated with the type of the arriving item. Since the span of the support of the random time is bounded by $L$, the support of the random packing is ``narrow''. This allows us a graceful increase in suboptimality. This argument is similar in spirit to the one carried out by \cite{Neely2009} in a queueing control setting where the environment process is driven by a Markov chain. However, there the author considers a deterministically delayed Lyapunov function to allow the environment at time $t$ to ``de-correlate'' with the state of queues at time $t-L$, and then uses the fact that state at time $t$ is close to the state at time $t-L$.

As we mentioned earlier, Theorem~\ref{thm:adversarial_smoothed} gives a family of bounds, one for each choice of $\epsilon, L$ and $L$-bounded fractional partition $\pi$. We do not discuss optimizing the bound over partitions $\pi$ as this will depend on the particular instance, but make two observations: First, since $\Pi(L_1,T) \subset \Pi(L_2, T)$ for $L_1 < L_2$, for any setting of $\epsilon$ as the smoothing window bound $L$ is increased from $\mO(1)$ to $o(1/\epsilon)$ the first term $\sum_t \hat{b}_{\pi,t }$ for the optimal partition $\pi \in \Pi(L,T)$ is non-increasing in $L$. However this improvement comes at the cost of an increased value for the second term $9T \epsilon L$ which is increasing in $L$. Second, while $L$ and $\pi \in \Pi(L,T)$ are purely part of analysis, the choice of $\epsilon$ is part of Algorithm~\ref{alg:PDexp_level} and controls the achievable family of bounds through the constraints $L < \frac{1}{\epsilon}$. A smaller $\epsilon$ thus allows smoothing over larger windows, but comes at a cost of $\frac{3 B}{\epsilon}$ in the performance bound in Theorem~\ref{thm:adversarial_smoothed}.

Returning to our \textbf{example} from the beginning of this Section for illustration, Theorem~\ref{thm:adversarial_smoothed} gives the following guarantees:
\begin{enumerate}
\item Case $\epsilon = \Theta \left(\frac{1}{\sqrt{T}} \right)$ : $\expct{N^{\PDexp}_T} \leq 0.25 T + \mO(T^{3/4})$. \\
Here $0.25 = b(\bar{\bF})$ and hence $\expct{N^{\OPT}_T} \geq 0.25 T$.  
To apply the Theorem, we need to decide the value of $L = o(1/\epsilon)$ as well as a specific $L$-bounded fractional partition. A choice of $L=4T^{1/4}$ allows us to average over the distributions in each phase to get $\hat{F}_{\pi,t} = \bar{\bF}$ for all $t \in [T]$. For the latter, we will use the blocked partitioning scheme mentioned earlier. Substituting in Theorem~\ref{thm:adversarial_smoothed} we get the bound mentioned above.
\item Case $\epsilon$ can be modified: $\expct{N^{\PDexp}_T } \leq 0.25 T + \mO(T^{5/8})$ \\
The optimal choice of $L$ remains $4 T^{1/4}$, and given this the optimal $\epsilon$ to minimize the upper bound in Theorem~\ref{thm:adversarial_smoothed} is $\epsilon = \mO(T^{-5/8})$. 
\end{enumerate}




\subsection{Locally adversarially perturbed {\it i.i.d.} sequences}
\label{sec:ni-i-d}

\textbf{Model: } Let $\mathbf{Y} =  \{ Y_1, \ldots, Y_T\}$ be an i.i.d. sequence of item types generated from $F$. Let $\{\mF_t\}$, $\mF_t = \sigma(Y_1, \ldots, Y_t)$, be the filtration generated by the process $\mathbf{Y}$. An adversary applies a permutation $\mu$ to $Y$ before presenting $\widetilde{\mathbf{Y}} = \{\widetilde{Y}_1,\ldots, \widetilde{Y}_T\} = \{Y_{\mu(1)}, \ldots, Y_{\mu(T)} \}$ to the online packing algorithm. We assume the following constraints on the adversary's choice of $\mu$:
\begin{enumerate} 
\item {\bf $L$-lookahead:} The event $\{\mu(k) = j \} $ is in $\mF_{j+\frac{L}{2}}$,
\item {\bf $L$-local perturbation:} $ \forall k , \ k-\frac{L}{2} \leq \mu(k) \leq k+\frac{L}{2}$. 
\end{enumerate}
Operationally, we can think of the adversary as a bounded delay, bounded buffer queueing system: the system is fed the sequence $Y_1, Y_2, \cdots $ and allowed a buffer of at most $L/2$ items. When presented with an item $Y_t$, the queue first emits zero or more items from its buffer, and then adds $Y_t$ to the buffer. The queue is also constrained in terms of maximum ``delay'' : an item $Y_t$ can not be overtaken by more than $L/2$ items arriving after it. After seeing $Y_T$, all remaining items in the buffer must be emitted in some order.

\begin{theorem}
\label{thm:adv_perturbed}
For the $L$-lookahead, $L$-local perturbation adversarial model, the expected number of bins used in packing the sequence $\widetilde{\mathbf{Y}}$ by Algorithm~\ref{alg:PDexp_level} is upper bounded by
\[ \expct{ N^{\PD}_T } \leq b(F) \cdot T +  T \kappa \epsilon \left(L + \frac{3}{2} \right) + \frac{B \kappa }{\epsilon} , \]
where $\epsilon_t = \epsilon$ and $\kappa$ denote the parameters of the penalized-Lagrangian function in Algorithm~\ref{alg:PDexp_level}, and $L, \epsilon, \kappa, B$ satisfy: $\epsilon L < 1$, and $L \leq \frac{1}{\epsilon} \log \frac{\kappa B}{B-1}$. 

As a corollary:
\begin{enumerate}
\item If $L=o(\sqrt{T})$ is unknown, then setting $\epsilon = \Theta((BT)^{-1/2})$: 
\[ \expct{N^{\PD}(T)}  \leq b(F) \cdot T + \mO(L \sqrt{BT} ). \]
\item If $L=o(T)$ is known, then setting $\epsilon = \Theta((BLT)^{-1/2})$:
\[ \expct{N^{\PD}(T)}  \leq b(F) \cdot T + \mO(\sqrt{BLT}). \]
\end{enumerate}
\end{theorem}

The proof of Theorem~\ref{thm:adv_perturbed} appears in Section~\ref{sec:proofs}. The main bound in the theorem resembles the bound of Theorem~\ref{thm:adversarial_smoothed}. Indeed, both theorems rely on the same Lemma. The difference is that the random times/smoothing windows of Theorem~\ref{thm:adversarial_smoothed} are replaced by $\mu^{-1}(t)$. By definition, the distribution at random time $\mu^{-1}(t)$ is $F$ (hence the term $b(F)$ in the Theorem), but these random times are not independent of the sequence $\mathbf{Y}$ anymore. 


%%%%%%%%%%%%%%%%%%%
% COMMENT BEGIN
%%%%%%%%%%%%%%%%%%%
\begin{comment}
\proof{Proof:} For the first part of the corollary, we apply Corollary~\ref{cor:fix_alpha} to a simple $L$-bounded fractional partition $\pi^*$ where $q_{iL+1} = q_{iL+2 }= \cdots = q_{(i+1)L} = \mbox{Unif}[\{ iL+1, \ldots, (i+1)L\}]$ for $i = 1, \ldots, \floor{\frac{T}{L}}$. That is, we partition the horizon into disjoint contiguous windows of length $L$, and our main goal is to optimize $L$ for use in the analysis (note the algorithm only depends on $\epsilon$ which we have fixed to $\Theta(T^{-1/2})$). Now for any $k$, the total variation norm of the smoothed distribution $\hat{F}_{\pi^*,k}$ and the true distribution $F$ is $\mO(W/L)$ and therefore  $\expct{\hat{b}_{\pi^*, k}} = b(F) + \mO(W/L)$. Applying Corollary~\ref{cor:fix_alpha}, we get 
\[ \expct{N^{PD}(T)} \leq b(F) \cdot T + \mO \left( \frac{WT}{L} + \frac{TL}{\epsilon}+ \frac{1}{\epsilon} \right)\]
This expression is minimized for $L = \Theta(T^{1/4}W^{1/2})$ giving the regret bound in the corollary statement.\\
Proof of the second case is similar, except when we optimize for $L$, we set $\epsilon = \Theta\left(\sqrt{\frac{1}{TL}} \right)$ as per Corollary~\ref{cor:vary_alpha}.
\Halmos \endproof
\end{comment}
%%%%%%%%%%%%%%%%%%%
% COMMENT END
%%%%%%%%%%%%%%%%%%%


%\begin{remark} Our analysis in Corollary~\ref{cor:adv_perturbed} is likely not tight. For $W=1$, the adversary is restricted to swapping some subset of adjacent pairs of the original sequence (after having seen the sequence). It would be surprising if this small perturbation causes the regret to jump from $\mO(\sqrt{T})$ to $\mO(T^{3/4})$. A likely line of attack might be to revert to the Online Mirror Descent (OMD) view of PD-exp (Section~\ref{sec:OMDinterp}), and then develop tighter regret analysis of OMD under a general correlation structure on gradients. While some analysis exists under mixing assumptions on the input sequence (\cite{agarwal2013generalization}), adversarial perturbations of $i.i.d.$ sequences do not belong to this class of inputs.\end{remark}

%In Section~\ref{sec:cornerpoint} we conjecture the existence of a complementary non-stationary guarantee to the one proved in this Section: If each $F_t$ lies in a certain set (Vertex-Dual distributions with a common unique vertex dual solution), then setting $\epsilon = \Theta(\log^{1+\beta} T)$ for any $\beta>0$ will result in expected regret $\mO(\log^{1+\beta} T)$ against the optimal offline packing.


==> tex/nonstationary_old_with_comments.tex <==
\section{Guarantees against non-$i.i.d.$ input sequences}
\label{sec:nonstationary}

As we mentioned in the introduction, one of our motivations behind designing distribution-oblivious online packing algorithms is that we hope they will be robust to non-stationary input sequences.
In this section, we prove guarantees of the Primal-Dual heuristic (Algorithm~\ref{alg:PDexp_level}) for two specific models of non-{\it i.i.d.} sequences:

\begin{enumerate}
\item Independent but not identically distributed: An arbitrary sequence of distributions $\{F_1, F_2, \ldots, F_T\}$  is fixed. The sequence $Y=\{Y_1, \ldots, Y_T\}$ is generated by sampling $Y_t$ from distribution $F_t$ independent of other $Y_j$'s. (Section~\ref{sec:i-ni-d})
\item Identically distributed but not independent: In this case we assume that first a sequence $\{Y_1,Y_2,\ldots, Y_T \}$ is generated by {\it i.i.d.} sampling from a distribution $F$, and then subsequently ``locally perturbed'' by an adversary with bounded look ahead. (Section~\ref{sec:ni-i-d})
\end{enumerate}

\subsection{Independent but not identically distributed model}
\label{sec:i-ni-d}

\textbf{Model: } An arbitrary sequence of distributions $\mathbf{F}= \{ F_1, F_2, \ldots, F_T \}$ is generated, possibly adversarially. Given $\mathbf{F}$, the sequence of item sizes $\mathbf{Y} = \{Y_1, Y_2, \ldots, Y_T\}$ is generated by sampling $Y_t$ from $F_t$ independent of $Y_{s}$ ($s \neq t$).

\noindent \textbf{Example:} Consider a packing instance with $B=9, J=3$. The sequence of distributions is $\mathbf{F} = \{  \underbrace{G_1, \ldots , G_1}_{T^{1/4}}, \underbrace{G_2, \ldots, G_2}_{T^{1/4}} , \ldots, \underbrace{G_{T^{3/4}}, \ldots , G_{T^{3/4}}}_{T^{1/4}} \}$. That is, the sequence $\mathbf{Y}$ has $T^{3/4}$ phases of length $T^{1/4}$ each, and within each phase $Y_t$ are {\it i.i.d}. Each $G_i$ is determined by sampling $p_2$ uniformly from the interval $[1/2,1]$ (independently for each $G_i$), and setting $p_3=1-p_2$.

\paragraph{A naive analysis : } We designed the instance above so that history-based learning is not useful -- the distribution changes after every $T^{1/4}$ times steps.
Let $F_t$ be the (random) distribution at time $t$. If we naively extend the proof of Theorem~\ref{thm:PDexp_fixed_epsilon}, we get that the number of bins used by PD-exp algorithm is bounded by:
\[ \expct{N^{PD}_{\{F_t\}}(T)} \leq \sum_{t=1}^T \expct{b(F_t)} + \sqrt{4BT}. \]    
Recall that $b(F)$ denotes the optimal value of $\mathbf{P_{1d-level}}$ giving the number of bins used per item in the optimal fractional packing. The value $b(F_t)$ is $\frac{1}{4}$ for $p_2 \geq \frac{3}{4}$, and $\frac{1}{3}-\frac{p_2}{9}$ for $p_2 \leq \frac{3}{4}$ (the distribution with $p_2 < 3/4$ is Bounded Waste, and with $p_2 > 3/4$ is Linear Waste). Therefore, $\expct{b(F_t)} = \frac{37}{144} \approx 0.257$. However, for the average distribution $p_2 = 3/4$, giving $b(\expct{F_t}) = \frac{1}{4} = 0.25$. Therefore we should expect the entire instance to be packed with sublinear waste, even though the distributions at a constant fraction of time steps are Linear Waste distributions. In this particular example, PD-exp indeed gives this desired result as we prove later in this Section.

\paragraph{Towards a more sophisticated analysis : } The reason the naively analysis yields a somewhat bad result is apparent from the proof of Theorem~\ref{thm:PDexp_fixed_epsilon}, where the change in Lagrangian at a given time $t$ is upper bounded by the change in Lagrangian due to a probabilistic policy $A_{F_t}$ which depends on the distribution from which the item at time $t$ is generated. Hence the term $\expct{b(F_t)}$ in the upper bound given above. To get a bound closer to $b(\expct{F_t})$ we would like to pretend that we are seeing a distribution closer to $\expct{F_t}$ -- in fact, even average of $\log T$ of the $G_i$ distributions gives a Bounded Waste distribution with high probability. Thus it is not sufficient to bound the change in Lagrangian at a {\it deterministic time} $t$, but we have to use {\it random times} $S_t$ whose distributions are smeared out enough so that the average item size distribution at any random time $S_t$ is ``nicer'' -- that is, has small $b(F_{S_t})$. Since $b(\cdot)$ is convex function, more smearing is desirable, but as we will see when we analyze random times based penalized-Lagrangian, there are trade-offs.

\subsubsection{Analysis}
As we mentioned, the crux of analysis is to calculate the change in Lagrangian at a random time so that the ``smoothed'' item size distribution at this random time has a smaller objective function value than at a deterministic time. Therefore, we need to define a collection of $T$ distributions for $T$ random times $(S_1, \ldots, S_T)$ which must satisfy the condition that the total change in Lagrangian over $\{1,\ldots, T\}$ equals the total change in Lagrangian over $\{S_1, \ldots, S_T\}$. It turns out we do not need the joint distributions of these $T$ random times but only their marginals. Towards this, we begin by defining what we call \emph{$L$-bounded fractional partition} of the time horizon $[T]$.

\begin{definition}[$L$-bounded fractional partition] A collection $\pi = \{ q_1, q_2, \ldots, q_T \}$ of $T$ probability measures, each with support on $[T]$ is called an $L$-bounded fractional partition of the time horizon $\{1,2,\ldots, T\}$ if it satisfies:
\begin{enumerate}
\item {\bf Bounded $L$-Support:} For all $u \in [T]$, $\max \{u : q_t(u)>0 \}-\min\{u : q_t(u)>0\} \leq L-1 $
\item {\bf Unit coverage:} For all $u \in [T]: \ \sum_t q_t(u) = 1$
\end{enumerate}
Let $\ell_t = \min\{u: q_t(u) > 0\}$ denote the earliest time $u$ in the support of $t$th window, and without loss of generality assume the windows are indexed so that $\ell_t$ is non-decreasing in $t$. Let $\Pi(L,T)$ denote the set of all $L$-bounded fractional partitions of $[T]$.
\end{definition}

See Figure~\ref{fig:partition_example} for an illustration. In words, window $t$ is defined by a probability measure $q_t$ on $\{1,\ldots, T\}$ which gives the distribution of random time $S_t$ (which we will interchangeably also call the $t$th smoothing window). The $L$-boundedness condition says that no smoothing window can have support on time instants more than $L$ apart, and the distribution for each time instant $t$ is completely partitioned across the $T$ windows in $\pi$. We will assume that the partition is deterministic, that is independent of $\{Y_1,\ldots, Y_T\}$. Indeed, the simplest example is where $q_{iL+1} = q_{iL+2} = \cdots = q_{(i+1)L} = \mbox{Unif}\{iL+1,iL+2, \ldots, (i+1)L\}$, $i=1,\ldots, \frac{T}{L}$.

\begin{figure}[ht!]
\centering
\includegraphics[width=5.5in]{partition}
\caption{An illustration of $L$-bounded fractional partitions of $[T]=\{1,2,\ldots,T\}$.}
\label{fig:partition_example}
\end{figure}

\begin{definition} Given an $L$-bounded fractional partition $\pi = \{q_t\}_{t\in [T]}$, the $t$th \emph{smoothed item size distribution} is defined to be:
\begin{align}
\hat{F}_{\pi, t} \triangleq \sum_{u=1}^T q_t(u) F_t 
\end{align}
Denote the optimal bin rate of $\mathbf{P_{1d-level}}$ with distribution $\hat{F}_{\pi, t }$ by $\hat{b}_{\pi, t}$.
\end{definition}

We are now ready to state our main result of this section.

\begin{theorem} \label{thm:adversarial_smoothed}
Consider the independent but non-identical arrival model described above with a packing horizon of $T$ items. 
%For a given window size $L$, define the \emph{$L$-smoothed arrival distribution} at time $k$ conditioned on $\mathcal{F}_t$ as:
%\[ \hat{F}_{L,k|t} \doteq  \expct{ \left. \frac{1}{L} \sum_{m=k}^{k+L-1} F_m  \right| \mathcal{F}_t} \]
%Denote the optimal bin-rate of the bin packing LP for $\hat{F}_{L,k|t}$ by $\hat{b}_{L,k|t}$. For succinctness, $\hat{b}_{L,k} \doteq \hat{b}_{L,k|0}$.
Let $\epsilon$ and $\kappa$ denote the parameters of the penalized-Lagrangian function in Algorithm~\ref{alg:PDexp_level}. 

If $L, \epsilon, \kappa, B$ satisfy: $\epsilon L < 1$, and $L \leq \frac{1}{\epsilon} \log \frac{\kappa B}{B-1}$, then for all $\pi \in \Pi(L,T)$, the expected number of bins used in packing the sequence $\mathbf{Y}=\{Y_1,\ldots, Y_T\}$ by Algorithm~\ref{alg:PDexp_level} is upper bounded by
\[ \expct{ N^{PD}(T) } \leq \sum_{t=1}^T \hat{b}_{\pi,t} +  T \kappa \epsilon \left( \frac{2L+3}{4} \right) + \frac{B \kappa }{\epsilon} . \]
\end{theorem}

The proof of Theorem~\ref{thm:adversarial_smoothed} appears in Appendix~\ref{sec:proofs}.
The main idea, again, is to calculate the change in the Lagrangian over a random time distributed according to the measure $q_k$. We can view this as calculating the change in Lagrangian in a single time step with item size distribution being the smoothed distribution $\hat{F}_{\pi,k}$ but where the packing seen by the arriving job is random, and potentially correlated with the type of the arriving item. Since the support of the random time is bounded by $L$, the support of the random packing is ``narrow''. This allows us a graceful increase in suboptimality. This argument is similar in spirit to the one carried out by \cite{Neely2009} in a queueing control setting where the environment process is driven by a Markov chain. However, there the author considers a deterministically delayed Lyapunov function to allow the environment at time $t$ to ``de-correlate'' with the state of queues at time $t-L$, and then uses the fact that state at time $t$ is ``$L$-close'' to the state at time $t-L$.

Theorem~\ref{thm:adversarial_smoothed} gives a family of bounds: For any setting of $\epsilon$, as the smoothing window bound $L$ is increased from $\mO(1)$ to $o(1/\epsilon)$ the first term $\sum_t \hat{b}_{\pi,t }$ is non-decreasing since the objective function $b(F)$ in $\mathbf{P_{1d-level}}$ is a convex function of $F$. Returning to our \textbf{example} from the beginning of this Section, Theorem~\ref{thm:adversarial_smoothed} gives the following guarantees:
\begin{enumerate}
\item Case $\epsilon = \Theta \left(\frac{1}{\sqrt{T}} \right)$ : $\expct{N^{PD}(T)} \leq 0.25 T + \mO(T^{5/6})$. \\
Here $0.25 = b(\expct{F_t})$, the offline optimal value of number of bins per item.  To apply the Theorem, we need to decide what value of $L = o(1\epsilon)$ gives the optimal regret. Setting $L = T^{1/4} \cdot k $ (i.e., we want to smooth $k$ phases), $\expct{\hat{b}_{\pi,t}} = 0.25 + \mO(\frac{1}{\sqrt{k}})$. The value of $k$ that minimizes the bound in Theorem~\ref{thm:adversarial_smoothed} is $k = \mO(T^{1/6})$ or $L = \mO(T^{5/12})$ giving the above bound.
\item Case $\epsilon$ can be modified: $\expct{N^{PD}(T) } \leq 0.25 T + \mO(T^{13/16})$ \\
The optimal choice of $\epsilon, L$ to minimize the upper bound in Theorem~\ref{thm:adversarial_smoothed} is $\epsilon = \mO(T^{-13/16}), L = \mO(T^{5/8})$. 
\end{enumerate}




\subsection{Locally adversarially perturbed {\it i.i.d.} sequences}
\label{sec:ni-i-d}

\textbf{Model: }

\textbf{Example: }


\subsection{Results }
\label{sec:noniid_analysis}

\varun{ {\bf Motivation:} Assume the items were arriving after a preprocessing step; perhaps a queueing system where a priority scheduling rule might reorder jobs so that the output is not i.i.d. anymore; however rescheduling only happens withing busy period, but due to history there may be a long range dependence on how the scheduler reorders jobs.}

\varun{ {\bf New nonstationary model:} Let $\Omega := [J]^T$ be the space of lenth $T$ sequences of item types. We assume that the item size sequence $\{Y_1, \ldots, Y_T\} \in \Omega$ is generated according to an arbitrary measure $\mu$ on $\Omega$. This defines a probability space (triple) $(\Omega, 2^{\Omega}, \mu)$. The sigma algebras $\F_t := \sigma(\{Y_1,\ldots, Y_t\})$ define a filtration, with $\F_0 = \{\emptyset, \Omega\}$. \\
Define an independent probability space $([0,1], \mathcal{B}, \nu)$, which defines the product space $(\Omega \times [0,1], 2^{\Omega} \times \mathcal{B}, \mu \times \nu) := (\Psi, \mathcal{B}_{\Psi}, \mu_{\Psi})$. Define $\mu_{\Psi}$ measurable random variables $\{S_1, \ldots, S_T\} $ with each $S_k$ taking values in $[T]$ such that:
\begin{enumerate}
\item {\bf Coverage:} $S_i \neq S_j$ for $i \neq j$, $\mu_\Psi$ a.s. (equivalently $\{S_1, \ldots, S_T\}$ define a permutation of $[T]$)
\item {\bf Bounded $L$-support:} Define 
$\ell_k := \min\{t : \mu_\Psi( S_k = t) >0 \} $
 and 
$u_k := \max\{t : \mu_\Psi( S_k = t) >0 \} $. Then, $u_k - \ell_k \leq L-1$
\end{enumerate}
Example 1: Adversarially perturbed input. First an i.i.d. sequence $\{X_1,\ldots, X_T\}$ is generated according to the product measure $\mu_0 = F\times \cdots \times F$. The an adversary randomly permutes this sequence to generate $\{Y_{1}, \ldots , Y_T\}$ possibly using extra randomness $Z$ which we without loss of generality assume to be an independent $Unif[0,1]$ random variable. We further impose the constraint that the adversary does not move any item more than $w$ position from its original position. Therefore, the permutation $\sigma = f(\{X_1, \ldots, X_T\}, Z)$ is a $\mu_0 \times \mu_Z$ -measurable (is this the right notation?) random element such that $Y_{\sigma(k)} = X_j$. Now defining $S_k = \sigma(k)$, the above two conditions are satisfied with $L=w$. \\
\ \\
Analysis: Prove concentration bound for the empirical distribution in each window -- focus on the event where empirical distributions are in the good ball. Now empirical distribution is roughly independent of the history a.s. on this event.  
 }

\varun{ {\bf Examples:}
\begin{enumerate}
\item  Adversarial perturbation 
\item Suppose $B=9$. Adversary at time $t$ picks a distribution on $\{2,3\}$ with $p_2$ sampled uniformly from $[0,1]$. No -- picking a $p_2$ and tossing a coin with this probability is the same as tossing a coin with the average $p_2$.
\[ \prob{X_H=1} =  \]
 Need at least 3 items to make this interesting, or that $p_2$ forms a Markov chain 
\end{enumerate}
}

We first formally define the model and notation for non-stationary sequence generation process:\\
\textbf{Non-stationary sequence model:} We will assume that the item size sequence $Y = \{Y_1, Y_2, \ldots, Y_T\}$ is generated from an arbitrary probability measure $\mu$ on $[J]^{T}$. An equivalent view is the following: At time $t$, Nature samples an item type $Y_t$ from distribution $F_t$ that is a deterministic function of the history of samples generated: $F_t = f_t(Y_1, \ldots, Y_{t-1})$. Let $ \left\{ \mathcal{F}_t \right\}$ denote the filtration generated by $\{ Y_1, \ldots, Y_t \}$ where as is usual $\mathcal{F}_0 = \{\emptyset, \Omega\}$. Therefore, $F_{t|0} \triangleq [F_t | \F_0]$ is a random distribution. Let
\begin{align*}
b_{t|0} = \expct{b(F_{t|0}) | \F_0}\ , \qquad  w_{t|0} = \expct{w(F_{t|0}) | \F_0}
\end{align*}
denote the expected bins per item and waste per item, respectively, under the random distribution $F_{t|0}$. \\
{\bf Example 1:} $Y = \{Y_1,\ Y_2, \ldots, Y_T\}$ is an \emph{i.i.d.} sequence with distribution $F$. In this case $\mu$ is the product measure $ F \times F \cdots \times F$. The random distribution $F_{t|0}$ is degenerate and equals $F$ with probability 1. \\
{\bf Example 2:} $Y = \{Y_1,\ Y_2, \ldots, Y_T\}$ is a sequence of independent but not identically distributed item sizes. In this case $\mu$ is the product measure $ F_1 \times F_2 \cdots \times F_T$. The random distribution $F_{t|0}$ is degenerate and equals $F_t$ with probability 1. \\
{\bf Example 3:} Let $Y=\{Y_1, \ldots, Y_T\}$ with  $Y_t \in \{2,3\}$ be generated as follows: define distribution $G = \{p_2=1/3, p_3 = 2/3\}$ and distribution $H = \{p_2 = 3/4, p_3 = 1/4\}$. With probability $1/2$, nature generates $Y$ from product measure $G \times G \cdots \times G$, and otherwise from product measure $H \times H \cdots \times H$. The random item size distribution $F_{t|0}$ is $G$ with probability $1/2$ and $H$ with probability $1/2$. Further, $b_{t|0} = \frac{b(G)+b(H)}{2} = \frac{ 8/27 + 1/4}{2}$, and $w_{t|0} = \frac{w(G) + w(H)}{2}=0$.

From the proof of Theorem~\ref{thm:PDexp_fixed_epsilon}, it is easy to obtain the following corollary: 
%Let the item at time step $t$ be generated from an arbitrary distribution $F_t$ chosen by an adversary, possibly after observing the packing decisions in the first $(t-1)$ time steps. If the optimal bin-rate (solution of $\mathbf{P_{conf}}$) for distribution $F_t$ is $b_t$ then the  PD-exp algorithm achieves: $ \expct{N_{\{F_t\}}^{PD}(T) } \leq \sum_{t=1}^T b_t + \mO(\sqrt{T}) $.
\begin{align*}
\expct{N^{PD}_{\mu} | \F_0} & \leq \sum_{t=1}^T b_{t|0} + \mO(\sqrt{T}) , \\
\expct{W^{PD}_{\mu} | \F_0} & \leq \sum_{t=1}^T w_{t|0} + \mO(\sqrt{T}) .
\end{align*}

For example, if Nature generates a non-stationary sequence under the constraint that for all $t$, the support of $F_t$ is restricted to distributions $F$ with waste $w(F)=0$, then PD-exp algorithm packs this non-stationary instance with waste $\mO(\sqrt{T})$, and hence the regret is $\mO(\sqrt{T})$ compared to the optimal offline packing.

However, the above guarantee is rather weak as shown by the following example: Consider the case where $B=3$, and $Y = \{ 1, 2, 1, 2, \ldots \} $. In this case $F_{t|0}$ is degenerate distribution $\{p_1=1\}$ if $t$ is even, and $\{p_2=1\}$ if $t$ is odd. The optimal bin-rate of the former distribution is $1/3$ bin/item and for the latter is $1$ bin/item, giving an average of $2/3$. However, it is conceivable that we should be able to achieve the hindsight optimal bin-rate of $1/2$ given the benign nature of input. As we show, we indeed have such a stronger guarantee against a \emph{smoothed} input sequence, albeit at a slightly worse additive suboptimality. In fact, we will prove a family of bounds parametrized by the size of the smoothing window, which hold simultaneously for PD-exp.

%\begin{remark} We could allow the adversary to sample items based on the actions of the PD algorithm until time $t-1$, since the PD algorithm is deterministic and therefore the adversary could simulate the actions of the PD algorithm. However, for randomized algorithms, we want the algorithm to have access to private randomness. Further, the adversarial model above allows analysis of algorithms with lookahead window of $L$ by forcing the adversary to commit to the next $L$ time steps, although we do not perform this analysis here. \end{remark}
 


\begin{corollary}  
\label{cor:fix_alpha}
If $\epsilon=\Theta(T^{-1/2})$ is fixed, then for $L = O(T^{c})$ with any $c<\frac{1}{2}$: 
\[  \expct{N_\mu^{PD}(T) } \leq \min_{\pi \in \Pi(L,T)} \left[ \sum_{k=1}^T \hat{b}_{\pi, k} \right] + O(T^{\frac{1}{2}+c}). \]
\end{corollary}

\begin{corollary}
\label{cor:vary_alpha}
If the size of the desired smoothing window is given as $L = \Theta(T^{c})$  ($0 \leq c < 1$), then choosing $\epsilon = \Theta(T^{-\frac{1+c}{2}})$:
\[ \expct{N_\mu^{PD}(T) } \leq \min_{\pi \in \Pi(L,T)} \left[ \sum_{k=1}^T \hat{b}_{\pi,k}  \right] + O(T^{\frac{1+c}{2}}). \]
\end{corollary}

Corollary~\ref{cor:fix_alpha} again gives a family of bounds parametrized by $L$ for a fixed $\epsilon$, while Corollary~\ref{cor:vary_alpha} dictates an optimal choice of $\epsilon$ given $L$ to minimize the regret term. corollary~\ref{cor:fix_alpha} implies that for the input sequence $Y=\{1,2,1,2,\cdots\}$, the PD-exp algorithm as-is gives an $\mO(\sqrt{T})$ regret compared to offline optimal packing.

The following is a further application of the above results to \emph{almost-stationary sequences}.

\varun{TODO: Need to be more formal in arguing that $\hat{F}_{\pi^*,k|t}$ is close to $F$, and therefore even when we condition on $\F_0$, we get something close to $b(F)$. Essentially, we want to first cast the adversarial perturbation model into the Non-stationary sequence model we defined earlier, and be more formal.}

\begin{corollary}[Local adversarially perturbed input]
\label{cor:adv_perturbed}
Let $Y =  \{ Y_1, \ldots, Y_T\}$ be an i.i.d. sequence of item types generated from $F$. Consider an adversary who applies a permutation $\sigma$ (possibly a function of $Y$) to $Y$ before presenting $\tilde{Y}= \{Y_{\sigma(1)}, \ldots, Y_{\sigma(T)} \}$ to the online packing algorithm. We assume the adversary is constrained in his choice of $\sigma$ as follows:  $ \forall k , \ k-\frac{W}{2} \leq \sigma(k) \leq k+\frac{W}{2}$. 
\begin{enumerate}
\item If $W=o(\sqrt{T})$ is unknown, then setting $\epsilon = \Theta(T^{-1/2})$ (that is, $L = T^{1/4}W^{1/2}$) 
\[ \expct{N^{PD}(T)}  \leq b(F) \cdot T + \mO(T^{3/4} W^{1/2}). \]
\item If $W=o(T)$ is known, then setting $\epsilon = \Theta(T^{-2/3}W^{-1/3})$ (that is, $L = T^{1/3}W^{2/3}$):
\[ \expct{N^{PD}(T)}  \leq b(F) \cdot T + \mO(T^{2/3} W^{1/3}). \]
\end{enumerate}
\end{corollary}
\proof{Proof:} For the first part of the corollary, we apply Corollary~\ref{cor:fix_alpha} to a simple $L$-bounded fractional partition $\pi^*$ where $q_{iL+1} = q_{iL+2 }= \cdots = q_{(i+1)L} = \mbox{Unif}[\{ iL+1, \ldots, (i+1)L\}]$ for $i = 1, \ldots, \floor{\frac{T}{L}}$. That is, we partition the horizon into disjoint contiguous windows of length $L$, and our main goal is to optimize $L$ for use in the analysis (note the algorithm only depends on $\epsilon$ which we have fixed to $\Theta(T^{-1/2})$). Now for any $k$, the total variation norm of the smoothed distribution $\hat{F}_{\pi^*,k}$ and the true distribution $F$ is $\mO(W/L)$ and therefore  $\expct{\hat{b}_{\pi^*, k}} = b(F) + \mO(W/L)$. Applying Corollary~\ref{cor:fix_alpha}, we get 
\[ \expct{N^{PD}(T)} \leq b(F) \cdot T + \mO \left( \frac{WT}{L} + \frac{TL}{\epsilon}+ \frac{1}{\epsilon} \right)\]
This expression is minimized for $L = \Theta(T^{1/4}W^{1/2})$ giving the regret bound in the corollary statement.\\
Proof of the second case is similar, except when we optimize for $L$, we set $\epsilon = \Theta\left(\sqrt{\frac{1}{TL}} \right)$ as per Corollary~\ref{cor:vary_alpha}.
\Halmos \endproof

\begin{remark} Our analysis in Corollary~\ref{cor:adv_perturbed} is likely not tight. For $W=1$, the adversary is restricted to swapping some subset of adjacent pairs of the original sequence (after having seen the sequence). It would be surprising if this small perturbation causes the regret to jump from $\mO(\sqrt{T})$ to $\mO(T^{3/4})$. A likely line of attack might be to revert to the Online Mirror Descent (OMD) view of PD-exp (Section~\ref{sec:OMDinterp}), and then develop tighter regret analysis of OMD under a general correlation structure on gradients. While some analysis exists under mixing assumptions on the input sequence (\cite{agarwal2013generalization}), adversarial perturbations of $i.i.d.$ sequences do not belong to this class of inputs.
\end{remark}

In Section~\ref{sec:cornerpoint} we conjecture the existence of a complementary non-stationary guarantee to the one proved in this Section: If each $F_t$ lies in a certain set (Vertex-Dual distributions with a common unique vertex dual solution), then setting $\epsilon = \Theta(\log^{1+\beta} T)$ for any $\beta>0$ will result in expected regret $\mO(\log^{1+\beta} T)$ against the optimal offline packing.


==> tex/proofs.tex <==

\section{Optimality analysis of the Primal-Dual Algorithm} \label{sec:proofs}


\subsection{A simple potential function based proof of near optimality}
Recall that we cast our algorithm as the minimization of the following Lagrangian: Denote the number of level $h$ bins, $1 \leq h \leq B$, by $N_h$:
\begin{align*}
L(\mathbf{N}(t)) &= \underbrace{B \cdot N_B - (\mbox{total volume of jobs seen})}_{F_{A}(t)} + \epsilon \cdot \underbrace{\frac{1}{2} \sum_{h=1}^{B-1} N_h(t)^2}_{V_{A}(t)}
\end{align*}
We will call the first term ($F_{A}$) the primal objective function value and the second term ($V_{A}$) the potential function value for algorithm $A$.

We first note that we can bound the waste of any algorithm $A$ at time $t$ as 
\begin{align}
W_A(t) \leq F_A(t) + B \sum_{h=1}^{B-1} N_h(t)
\end{align}

\begin{claim}
For the Primal Dual algorithm, $ 0 \leq N_{h} \leq  \frac{B^2}{\epsilon}$, $1\leq h \leq B-1$.
\end{claim}
\begin{proof}
We can always choose to send an item to level 0 and pay a cost of at most $B$. Therefore, none of the $\gamma$ differences between and $h$ and $h-s_j$ grow larger than $B$. (In fact they should be bounded by $B$ because clearly for $h' = \max_j (B-s_j)$, $\gamma_{h'}<B$, because to increase it to $B$ we would have preferred sending item at this elevel over sending it to 0, which had a cost of at most B. Intuitively we can imagine $\gamma_0 \equiv B$, $\gamma_B \equiv 0$, and then the PD algorithm assigns based on minimizing the disparity. So the $\gamma$ should form a decreasing sequence. But this would need more careful arguing).
\end{proof}

The above claim implies that the waste due to partially filled bins is at most $\frac{B^4}{2\epsilon}$. Therefore we will now show that
\begin{align}
\expct{F_{PD}(T)} \leq \expct{F_{OPT}} + \epsilon T 
\end{align}
By choosing $\epsilon = \frac{1}{\sqrt{T}}$, we then establish additive $\sqrt{T}$ waste of the Primal-Dual algorithm. 

We first mention the proof steps at an abstract level and fill in the details subsequently. Since, the primal dual algorithm minimizes the increase in Lagrangian at each time step:
\begin{align*}
\Delta F_{PD}(t) + \epsilon \Delta V_{PD}(t) &\leq \Delta F_{OPT} + \epsilon \Delta V_{OPT}
\end{align*}

where all the deltas are given we start from the current state and $OPT$ is some algorithm which we use as the representative of the optimal algorithm. Taking a telescoping sum of the above inequality gives us:
\begin{align*}
F_{PD}(T) - F_{OPT}(T) & \leq \epsilon [ V_{OPT}(T)  -V_{OPT}(0) ] - \epsilon [V_{PD}(T) - V_{PD}(0)] \\
& \leq \epsilon(V_{OPT}(T) + V_{PD}(0))
\end{align*}
assuming $V$ is non-negative, which it usually is.

Intuitively this means that our algorithm performs well for the Lagrangian compared to $OPT$, but we really wanted the primal objective $F$ to be good. This happens if the OPT algorithm has not accumulated too much potential. Now for the bin packing problem, we would like to use the $A_F$ algorithm from the Sum-of-Squares paper as a probabilistic algorithm whose performance is close to OPT, and for which we know that $V_{A_F}(T) \leq  T$.

However, there is one place we overlooked things: the $\Delta F_{OPT}(t)$ and $\Delta V_{OPT}(t)$ are the changes given the current state of the PD algorithm. How do we then relate $\sum \Delta F_{OPT}$ and $\sum \Delta V_{OPT}$ to $F_{OPT}(T)$ and $V_{OPT}(T)$? For the $A_F$ algorithm there is no problem with $V_{A_F}$ since we know it increases by at most $1$ given \emph{any} configuration. We still need a way to relate $\Delta F_{OPT}$ to $\frac{F_{OPT}(T)}{T}$.

\begin{proposition}
Given an arbitrary packing $P$, the probability that $A_F$ packs an item to close a bin (create a level $B$ bin) is at most the probability that a random item in the perfect packing $P^*$ is on the top of its bin.
\end{proposition}
\begin{proof}
The proof is straightforward: For every bin $Y$ of $P^*$, $A_F$ first creates an ordering of items. Note that each of the items in $P^*$ arrive with equal probability. Now, if $A_F$ sees an item it maps to bin $Y$, then it can only create a level $B$ bin if it was the topmost item in the ordering. There is still a chance that it does not create a level $B$ bin because no bin of level $B-s$ exists.
\end{proof}

We haven't mentioned yet how to handle the case where $F$ is not perfectly packable: We simply look at the optimal packing $P^*$, and in any bin which is not perfectly packed, we meld the hole with any chosen item. When $A_F$ sees this item, it pretends that it sees a bigger item -- of size equal to the item plus the hole.

We thus have:
\begin{align*}
\Delta F_{PD}(t) + \epsilon \Delta V_{PD}(t) &\leq \Delta F_{A_F} + \epsilon \Delta V_{A_F}
\intertext{taking expectations:}
\expct{\Delta F_{PD}(t)} -\expct{\Delta F_{A_F}(t)} &\leq \epsilon \expct{\Delta V_{A_F}} - \epsilon \expct{ \Delta V_{PD}} \\
\intertext{Using the result of \cite{} that $\expct{\Delta V_{A_F}} \leq 1$,}
\expct{\Delta F_{PD}(t)} - [B \cdot p_F - \expct{s_F}] &\leq  \epsilon - \epsilon \expct{\Delta V_{PD}} \\
\intertext{Where $p_F$ is the rate at which OPT creates bins, and $s_F$ is the expected job size under $F$. Summing:}
\expct{F_{PD}(T)} - T \cdot W_F & \leq \epsilon T + \epsilon \expct{V_{PD}(0)}
\end{align*}
Where $W_F$ is optimal value of the waste LP.

By choosing $\epsilon = \Theta(\frac{1}{\sqrt{T}})$, we obtain additive $O(\sqrt{T})$ waste.

\textbf{Time-varying $\epsilon$} \\
In fact the above proof can be easily modified to show that when $\epsilon(t) = \frac{1}{\sqrt{t}}$, we still get $O(\sqrt{T})$ waste.

The result about the $N_h$ being bounded by $\frac{B^2}{\epsilon(T)}$ still holds.

We then have at time $t$:
\begin{align*}
\Delta F_{PD}(t) + \epsilon(t) \left( V_{PD}(t)-V_{PD}(t-1) \right) &\leq \Delta F_{OPT} + \epsilon(t) \left( V_{OPT}(t) - V_{OPT}(t-1) \right) 
\end{align*}

Taking a telescoping sum of the above inequality gives us:
\begin{align*}
F_{PD}(T) - \sum_t \Delta F_{OPT}(t) & \leq \sum_{t=1}^{T} \epsilon(t) [ V_{OPT}(t)  -V_{OPT}(t-1) ] \\
& \quad + \sum_{t=1}^{T-1} V_{PD}(t) (\epsilon(t+1) - \epsilon(t)) +\epsilon(1) V_{PD}(0) - \epsilon(T) V_{PD}(T) 
\intertext{and taking expectations, and noting that $\epsilon(t)$ is decreasing:}
\expct{F_{PD}(T)} - T \cdot W_F & \leq \sum_{t=1}^{T} \epsilon(t) + \epsilon(1) V_{PD}(0) - \epsilon(T) V_{PD}(T)  \\
& \leq 1 + \int_{1}^T \epsilon(t) dt + \epsilon(1) V_{PD}(0)  \\
\intertext{and choosing $\epsilon(t) = 1/\sqrt{t}$}
& \leq 2 \sqrt{T} + V_{PD}(0)
\end{align*}

\textbf{Optimizing $\epsilon(t)$} : We want $\epsilon(t) = \frac{K}{\sqrt{t}}$ for some $K$. Here we give some guidelines on choosing $K$. Roughly, we expect $N_h \approx \frac{h}{\epsilon}$, which would imply that the waste due to partially filled bins is 
\begin{align*}
\frac{1}{\epsilon} \sum_{h=1}^{B-1} h (B-h) &= \frac{\sqrt{T}}{K} \left( B \sum_{i}^{B-1} h - \sum_{i}^{B-1} h^2 \right) \\
& = \frac{\sqrt{T}}{K} \left( \frac{B^2(B-1)}{2} - \frac{(B-1)B(2B-1)}{6} \right)
\sim \frac{B^3}{6K} \sqrt{T}.
\end{align*}
The potential argument yields a further waste of $2K\sqrt{T}$. The sum is minimized when $K = \sqrt{\frac{B^3}{12}}$, and we get $O(\sqrt{B^3 T})$ additive waste.

(Without the above assumption, we have a waste that is $\sqrt{T} \left( \frac{B^4}{2\kappa} + 2\kappa \right) $, which can be minimized by choosing $\kappa = \frac{B^2}{2}$ and gives $\sqrt{B^4 T}$ additive waste).

\subsubsection{Proof using exponential penalty function}
Our Lagrangian is:
\begin{align}
L(\mathbf{N}(t)) &= \underbrace{\sum_{h=1}^{B-1} (B-h) N_h(t) }_{F_A(t)} + \underbrace{ \frac{1}{\epsilon_1} \sum_{h=1}^{B-1} e^{-\epsilon_2 N_h(t) } }_{V_A(t)}
\end{align}

The change in Lagrangian on a move is:
\begin{align*}
\Delta L(\mathbf{N}) & \leq \sum_{h=1}^{B-1} (B-h) \sgn{\Delta N_h}  -\sum_{h=1}^{B-1} e^{-\epsilon_2 N_h } \left[ \frac{\epsilon_2}{\epsilon_1} \sgn{\Delta N_h} - \frac{\epsilon_2^2}{\epsilon_1}  \right]
\end{align*}
Our goal is to find a policy for which the change in primal as well as potential term is small. The first means that the policy we want should open a new bin with a probability not larger than the long run rate, given any state. Small increase in the potential term means that we prefer creating bins of some level rather than destroying them. 

%Consider that we start from the empty system. Then no matter what policy we choose, we must have $L(0) = \frac{B-1}{\epsilon}$, $L(1) = (B-s) - \frac{1}{\epsilon_1}\left( (B-2) + e^{-\epsilon_2} \right) $, and therefore, $L(1) - L(0) = (B-s) - (\frac{\epsilon_2}{\epsilon_1} - \frac{\epsilon_2^2}{2! \epsilon_1} + \frac{\epsilon_2^3}{3!\epsilon_1} - \cdots ) $. For a perfectly packable distribution, we want this to be less than $(0 + \Theta(\epsilon))$. This suggests $\epsilon_2 > B \cdot \epsilon_1$, and then the increase in primal is dwarfed by the decrease in potential function.

We can again use exactly the $A_F$ policy. We first recall the policy: Given a bin $Y$ in the perfect packing $P^*$ and the current arbitrary packing $P$, we first find an ordering $y_1,y_2,\ldots, y_{|Y|}$ of the items in $Y$, and a threshold index $last(Y), \ 0 \leq last(Y) < |Y|$, such that if we set $S_i \equiv \sum_{j=1}^{i} s(y_j)$, then:
\begin{itemize}
\item $P$ has partially filled bins with each level $S_i$, $0 \leq i \leq last(Y)$
\item $P$ has no partially filled bins with level $S_{last(Y)} + s(y_i)$ for any $i > last(Y)$
\end{itemize}

Below we show the change in Lagrangian for various cases, conditioned on the arrival happening from bin $Y$ of perfect packing and getting mapped to index $j$ in the ordering:
\begin{itemize}
\item Case $j > last(Y)$ : all these items are sent to a partial full bin at level $S_{last(Y)}$ (or 0 if $last(Y)=0$). This seems like a bad case because we kill bins of some level with a higher probability than we create it and that increases our potential function (unlike for SS potential). Also, if $last(Y)=0$, then we open new bins at a probability higher than OPT. However, the crucial observation is that in the process we create bin of some level which does not exist yet. This causes sufficiently large drop in potential to completely annihilate the increase in primal term or the potential term for $S_{last(Y)}$. 
\begin{itemize}
\item Subcase $last(Y) = 0$ : In this case the change in Lagrangian is upper bounded by:
\begin{align*}
\Delta L &\leq -s(y_j) + B + \frac{1}{\epsilon_1} (e^{-\epsilon_2} - 1) \\
& = -s(y_j) + B - \frac{\epsilon_2}{\epsilon_1} \left(1 - \frac{\epsilon_2}{2!} + \frac{\epsilon_2^2}{3!} - \ldots \right) \\
\intertext{for $\epsilon_2 < 1$:}
& \leq  -s(y_j) + B - \frac{\epsilon_2}{\epsilon_1} \left( 1 - \frac{\epsilon_2}{2}  \right) \\
& = -s(y_j) + B - \frac{\epsilon_2}{\epsilon_1} + \frac{\epsilon_2}{\epsilon_1} \cdot \frac{\epsilon_2}{2} \\
\intertext{and choosing $\epsilon_2 = B\epsilon_1$}
& = -s(y_j) +   \frac{B}{2} \epsilon_2
\end{align*}
\item Subcase $last(Y) > 0$ : In this case, we send an item to a level $ h = S_{last(Y)} > 0$ with $n_h > 0$ so there is no change in the objective function term, but the potential term increases by at most:
\begin{align*}
\Delta L &\leq -s(y_j) - \frac{1}{\epsilon_1} \left[ \left(1 - e^{-\epsilon_2} \right) - \left(e^{- n_h \epsilon_2} - e^{-(n_h-1) \epsilon_2 }\right)  \right] \\
& \leq -s(y_j)
\end{align*}
\end{itemize}
\item Case $ 1 \leq j \leq last(Y)$ : Exactly one of these items causes a new bin to open and increase the objective function term by $B-s(1)$, the others casuse the objective function term to change by $-s(y_j)$. We now focus on the change in potential function due to bins of level $S_1, \ldots, S_{last(Y)-1}$. We do not need to look at $S_{last(Y)}$ since $j=last(Y)$ only causes this number to increase and hence potential to fall, and we have already accounted for the effect of $j>last(Y)$ on the Lagrangian. 

Focusing on this set of items, the probability of the increase of $N_{S_i}$ is at least as much as the probability of decrease of $N_{S_i}$. Therefore, the expected change in the potential function due to level $S_i$ is at most (let $N_{S_i}=n$ before arrival of the tagged item):
\begin{align*}
\Delta V_i &  \leq \frac{1}{2\epsilon_1} \left[ \left( e^{-(n+1)\epsilon_2} - e^{-n \epsilon_2} \right)  + \left(e^{-(n-1)\epsilon_2} - e^{-n \epsilon_2} \right) \right] \\
&= \frac{e^{-n \epsilon_2}}{2\epsilon_1} \left[ e^{-\epsilon_2} + e^{\epsilon_2} - 2  \right] \\
&= \frac{e^{-n \epsilon_2}}{\epsilon_1} \left[ \frac{\epsilon_2^2}{2!} + \frac{\epsilon_2^4}{4!} + \frac{\epsilon_2^6}{6!} + \ldots  \right] \\
\intertext{for $0 < \epsilon_2 < 1$}
& \leq  \frac{\epsilon_2^2}{\epsilon_1}
\intertext{and further for $\frac{\epsilon_2}{\epsilon_1} = B$:}
& \leq  B \epsilon_2
\end{align*}
\end{itemize}

Now we look at the telescoping sum of changes in Lagrangian:
\begin{align*}
\Delta F_{PD}(t) + \Delta V_{PD}(t) &\leq \Delta F_{A_F} + \Delta V_{A_F}
\intertext{taking expectations:}
\expct{\Delta F_{PD}(t)} &\leq \expct{\Delta F_{A_F}(t)} + \expct{\Delta V_{A_F}} - \expct{ \Delta V_{PD}} \\
\intertext{or,}
\expct{\Delta F_{PD}(t)} & \leq [B \cdot p_F - \expct{s_F}] \leq  B \epsilon_2 - \expct{\Delta V_{PD}} \\
\intertext{Where $p_F$ is the rate at which OPT creates bins, and $s_F$ is the expected job size under $F$. Summing:}
\expct{F_{PD}(T)} & \leq T \cdot W_F + B T \epsilon_2 + \expct{V_{PD}(0)} \\
\intertext{or}
\expct{F_{PD}(T)} & \leq T \cdot W_F + B T  \epsilon_2 + \frac{B-1}{\epsilon_1} \\
\intertext{observing the conditions on analysis so far that $\epsilon_2 = B \epsilon_1$, if we choose $\epsilon_1 = \sqrt{\frac{1}{BT}}$ we get:}
\expct{F_{PD}(T)} & \leq T \cdot W_F + 2 \sqrt{B^3 T}
\end{align*}
Where $W_F$ is optimal value of the waste LP.

\textbf{Time-varying $\epsilon(t)$} \\
The proof carries through with minimal changes in the last step. The changes in the potential term of the PD algorithm do not telescope any more. In particular, the potential function keeps decreasing since $\epsilon(t)$ decreases. Instead of $V_{PD}(T) - V_{PD}(0)$, the sum of potential differences looks like:
\begin{align*}
\sum \Delta V_{PD}(t) &= (B+1) \sum_{h=1}^{B-1} \sum_{t=1}^{T} \frac{1}{\epsilon(t)} (e^{-\epsilon(t)n_h(t)} - e^{-\epsilon(t)n_h(t-1)}) \\
&=  (B+1) \sum_{h=1}^{B-1}\left[ \frac{e^{-n_h(T) \epsilon(T)}}{\epsilon(T)} - \frac{e^{-\epsilon(0)n_h(0)}}{\epsilon(0)} + \sum_{t=2}^{T-1} \left( \frac{1}{\epsilon(t)} e^{ \epsilon(t) n_h(t)} - \frac{1}{\epsilon(t+1)} e^{-\epsilon(t+1)n_h(t)} \right) \right] \\
\intertext{the last difference is minimized when $n_h(t) = 0$ to give}
& \geq   (B+1) \sum_{h=1}^{B-1}\left[  - \frac{e^{-\epsilon(0)n_h(0)}}{\epsilon(0)} + \sum_{t=2}^{T-1}\left( \frac{1}{\epsilon(t)} - \frac{1}{\epsilon(t+1)} \right) \right] \\
\intertext{and choosing $\epsilon(t) = \frac{1}{\sqrt{t}}$}
& \geq - (B+1)  \sum_{h=1}^{B-1}\left[  1  + \sum_{t=2}^{T-1} \frac{1}{2\sqrt{t}} \right] \\
& \geq - B(B+1) (1+\sqrt{T})
\end{align*}
which only gives us slightly worse waste ( a factor of $2$ perhaps), and we have to be careful to maintain $\epsilon_2 < 1$, so we can not start with $\epsilon_1 = \frac{1}{\sqrt{(B+1)t}}$.

\subsubsection{Proof using $\log$-barrier function}
Our Lagrangian is:
\begin{align}
L(\mathbf{N}(t)) &= \underbrace{\sum_{h=1}^{B-1} (B-h) N_h(t) }_{F_A(t)} + \underbrace{ \frac{1}{\epsilon} \sum_{h=1}^{B-1} \log \frac{1}{N_h(t)+1} + \frac{1}{\epsilon} \log{(t+1)} }_{V_A(t)}
\end{align}
The last term does not actually have any influence on the algorithm, but we may need it in the future (especially because it guarantees that the potential remains positive) so we mention it here. In subsequent analysis we may drop it.

The change in Lagrangian on a move is:
\begin{align*}
\Delta L(N) &= \sum_{h=1}^{B-1} (B-h) \sgn{\Delta N_h}  +  \frac{1}{\epsilon} \sum_{h=1}^{B-1} \log \frac{N_h(t)+1}{N_h(t+1)+1} + \frac{1}{\epsilon} \log{\frac{t+2}{t+1}}
\end{align*}

To perform similar analysis as until now, we have to tweak the $A_F$ policy a little bit. In particular, given the current packing $P$, it is not sufficient to look at levels for which we have partially filled bins or not. Instead, we need to look at levels for which we have more or less than a threshold $A$ number of bins:


Below we show the change in Lagrangian for various cases, conditioned on the arrival happening from bin $Y$ of perfect packing and getting mapped to index $j$ in the ordering:
\begin{itemize}
\item Case $j > last(Y)$ : all these items are sent to a partial full bin at level $S_{last(Y)}$ (or 0 if $last(Y)=0$). This seems like a bad case because we kill bins of some level with a higher probability than we create it and that increases our potential function (unlike for SS potential). Also, if $last(Y)=0$, then we open new bins at a probability higher than OPT. However, the crucial observation is that in the process we create bin of some level $h^*$ for which $N_{h^*} \leq A$ and this causes sufficiently large drop in potential to completely annihilate the increase in primal term or the potential term for $S_{last(Y)}$.\
\begin{itemize}
\item Subcase $last(Y) = 0$ : In this case the change in Lagrangian is upper bounded by (we drop the last term since it cancels on both sides eventually):
\begin{align*}
\Delta L &= -s(y_j) + B + \frac{1}{\epsilon} \log\frac{n}{n+1} \\
 &= -s(y_j) + B - \frac{1}{\epsilon} \log (1+\frac{1}{n})\\
& \leq -s(y_j) +B - \frac{1}{\epsilon} \log\left(1 + \frac{1}{A} \right) \\
& \leq -s(y_j) +B - \frac{1}{\epsilon } \cdot \frac{1}{2A}  \\
& \leq -s(y_j)
\end{align*}
for $\epsilon A \leq \frac{1}{2B}$.
\item Subcase $last(Y) > 0$ : In this case, we send an item to a level $ h = S_{last(Y)} > 0$ with $n_h > 0$ so there is no change in the objective function term, but the potential term increases by at most:
\begin{align*}
\Delta L &\leq -s(y_j) + \frac{1}{\epsilon} \left[ \log \frac{A}{A+1}  + \log \frac{n_h}{n_h-1}  \right] \\
& \leq -s(y_j)
\end{align*}
since $n_h > A$, be definition of $A_F$.
\end{itemize}
\item Case $ 1 \leq j \leq last(Y)$ : Exactly one of these items causes a new bin to open and increase the objective function term by $B-s(1)$, the others casuse the objective function term to change by $-s(y_j)$. We now focus on the change in potential function due to bins of level $S_1, \ldots, S_{last(Y)-1}$. We do not need to look at $S_{last(Y)}$ since $j=last(Y)$ only causes this number to increase and hence potential to fall, and we have already accounted for the effect of $j>last(Y)$ on the Lagrangian. We also remember for all these levels $N_{S_j} \geq A+1$.

Focusing on this set of items, the probability of the increase of $N_{S_i}$ is at least as much as the probability of decrease of $N_{S_i}$. Therefore, the expected change in the potential function due to level $S_i$ is at most (let $N_{S_i}=n$ before arrival of the tagged item):
\begin{align*}
\Delta V_i &  \leq  - \frac{1}{2 \epsilon} \left[  \log{\frac{n-1}{n}} + \log{\frac{n+1}{n}}  \right] \\
&= \frac{1}{\epsilon} \left(\frac{1}{2n^2} + \frac{1}{4n^4} + \frac{1}{6n^6} \cdots   \right)\\
& \leq \frac{1}{\epsilon} \cdot \frac{1}{n^2}
\end{align*}
for $ n \geq 2 $.
\end{itemize}

Now we look at the telescoping sum of changes in Lagrangian:
\begin{align*}
\Delta F_{PD}(t) + \Delta V_{PD}(t) &\leq \Delta F_{A_F} + \Delta V_{A_F}
\intertext{taking expectations:}
\expct{\Delta F_{PD}(t)} &\leq \expct{\Delta F_{A_F}(t)} + \expct{\Delta V_{A_F}} - \expct{ \Delta V_{PD}} \\
\intertext{or,}
\expct{\Delta F_{PD}(t)} & \leq [B \cdot p_F - \expct{s_F}] \leq  \frac{1}{\epsilon A^2} - \expct{\Delta V_{PD}} \\
\intertext{Where $p_F$ is the rate at which OPT creates bins, and $s_F$ is the expected job size under $F$. Summing:}
\expct{F_{PD}(T)} & \leq T \cdot W_F + \frac{T}{\epsilon A^2} \epsilon_2 + \expct{V_{PD}(0)} - \expct{V_{PD}(T)} \\
\intertext{Note that in this case, our potential function does become negative. While $V_{PD}(0)=0$, $V_{PD}(T)$ can be as small as $-\frac{B}{\epsilon} \log T $. Therefore,}
\expct{F_{PD}(T)} & \leq T \cdot W_F + \frac{T}{\epsilon A^2} + \frac{B}{\epsilon} \log{T} \\
\intertext{where we can choose $\epsilon, A$ subject to $A \geq 2$ and $\epsilon A \leq \frac{1}{2B}$. Choosing $A = \sqrt{\frac{T}{B \log T}}$ and $\epsilon = \frac{1}{2BA} = \sqrt{\frac{\log T}{4BT}} $ gives:}
\expct{F_{PD}(T)} & \leq T \cdot W_F + 4 \sqrt{B^3 T \log T } 
\end{align*}
Interestingly, $\log$-barrier (using current analysis) does not give us $\sqrt{T}$ waste but $\sqrt{T \log T}$ waste!

\subsubsection{Analysis for bounded waste distributions}
For the exponential penalty case, it would seem we need $\epsilon < \frac{1}{B}$, but is $\Theta(1)$ enough?

\subsection{Optimality analysis under departures}
\subsubsection{Inadequacy of the quadratic penalty Primal-Dual algorithm}
We first show that our first attempt of using quadratic penalty can give a very slow convergence rate. In particular, if we start with the items from a perfectly packable distribution in a worst case configuration with linear waste, then it can take $\Omega(\sqrt{\lambda})$ time until the waste become sublinear.

In fact, our example is the simplest possible. All our items are of size 1, and the number of items in the initial configuration are a sample from the Poisson distribution with mean $\lambda$. However, all our jobs are in bins where we have a hole of 1 unit at the bottom, and then the bins are packed until level $B$. The reason quadratic penalty algorithm fails is that we do not have any mechanism to reclaim the holes at the bottom until the bin empties, and this can take a long time.

To make this more formal, recall that our Lagrangian is $B \cdot N_B + \epsilon(\lambda) \sum_{h=1}^{B-1} N_h^2$, where $\epsilon(\lambda) = \Theta(\frac{1}{\sqrt{\lambda}})$.

Under the above settings, all our $N_h$ are $\Theta(\frac{1}{\epsilon}) = \Theta(\sqrt{\lambda})$. In fact, it is not hard to see that $N_h$ will be tightly concentrated around $\frac{B-h}{\epsilon}$ because of the Primal-Dual algrorithm. We choose some bin $Y$ in the initial configuration, and see its evolution. We call the bin to be in state $i$, $0\leq i \leq B-1$ if it has $B-1$ items of size 1 above the hole. Now, when the bin is in state $i$, there are $\Theta(\sqrt{\lambda})$ other bins also in state $i$. We want to say that this bin will actually become a state $i+1$ bin before it can lose another item.

However, the problem is that this bin stays in state $i$ for $\Theta(1)$ time (since the rate of creation and destruction of level $i<B-1$ bins is $\sqrt{\lambda}$?), except when $i=B-1$ (in which case, it stays in state $B-1$ for $\frac{1}{\sqrt{\lambda}}$ time.) Therefore, once a bin becomes a state $B-2$ bin, it can empty out in $\Theta(1)$ time.

However, we still have that for a bin in state $B-1$ in initial configuration, it will take $\Omega(\sqrt{\lambda})$ time to become empty. This is quite slow. This problem does not arise with exponential penalty function. If we start with a state which has linear waste, under exponential penalty, we reach (?) a state with sublinear waste in $O(1)$ time.

